Neural Network Approximators for Marginal MAP in Probabilistic Circuits

Probabilistic circuits (PCs) such as sum-product networks efficiently represent large multi-variate probability distributions. They are preferred in practice over other probabilistic representations such as Bayesian and Markov networks because PCs can solve marginal inference (MAR) tasks in time that scales linearly in the size of the network. Unfortunately, the maximum-a-posteriori (MAP) and marginal MAP (MMAP) tasks remain NP-hard in these models. Inspired by the recent work on using neural networks for generating near-optimal solutions to optimization problems such as integer linear programming, we propose an approach that uses neural networks to approximate (M)MAP inference in PCs. The key idea in our approach is to approximate the cost of an assignment to the query variables using a continuous multilinear function, and then use the latter as a loss function. The two main benefits of our new method are that it is self-supervised and after the neural network is learned, it requires only linear time to output a solution. We evaluate our new approach on several benchmark datasets and show that it outperforms three competing linear time approximations, max-product inference, max-marginal inference and sequential estimation, which are used in practice to solve MMAP tasks in PCs.

==> content/0-abstract.tex <==
\begin{abstract}
\eat{
 Probabilistic circuits (PCs) are efficient representations of joint probability distributions. Unlike generally structured intractable Bayesian networks (BNs) and Markov networks (MNs), PCs enable probabilistic queries like computing marginal probabilities (MAR) or finding the most probable explanations (MPE) to be answered efficiently in linear time. Unfortunately, akin to Bayesian Networks (BNs) and Markov Networks (MNs), tackling the task of marginal maximum-a-posteriori (MMAP) within these models continues to pose an NP-hard challenge. In recent times, deep neural networks have exhibited promising outcomes in addressing optimization problems, particularly those related to max-inference problems. Drawing inspiration from these insights, our proposal revolves around elevating the precision of MMAP computations within Probabilistic Circuits (PCs) through the incorporation of advanced neural network architectures. Leveraging how PCs concisely represent joint distributions, we devise a scalable loss function for the neural network such that given data, it \textit{learns} to answer MMAP queries over PCs optimally. By conducting thorough experimentation across diverse benchmark datasets, our study emphasizes the notable effectiveness of our approach in comparison to competing methodologies.}
 
 Probabilistic circuits (PCs) such as sum-product networks efficiently represent large multi-variate probability distributions. They are preferred in practice over other probabilistic representations such as Bayesian and Markov networks because PCs can solve marginal inference (MAR) tasks in time that scales linearly in the size of the network. Unfortunately, the most probable explanation (MPE) task and its generalization, the marginal maximum-a-posteriori (MMAP) inference task remain NP-hard in these models. Inspired by the recent work on using neural networks for generating near-optimal solutions to optimization problems such as integer linear programming, we propose an approach that uses neural networks to approximate MMAP inference in PCs. The key idea in our approach is to approximate the cost of an assignment to the query variables using a continuous multilinear function and then use the latter as a loss function. The two main benefits of our new method are that it is self-supervised and after the neural network is learned, it requires only linear time to output a solution. We evaluate our new approach on several benchmark datasets and show that it outperforms three competing linear time approximations, max-product inference, max-marginal inference and sequential estimation, which are used in practice to solve MMAP tasks in PCs.
\end{abstract}

 \eat{Unfortunately, just like BNs and MNs the marginal maximum-a-posteriori (MMAP) task remains NP-hard in these models. Recently, deep neural networks have shown promising results in solving optimization problems, specifically max-inference problems.}

==> content/1-intro.tex <==
\section{Introduction}\label{sec:intro}
Probabilistic circuits (PCs) \cite{choiProbCirc20} such as sum-product networks (SPNs) \cite{poon2011sum}, arithmetic circuits \cite{darwiche2003differential}, AND/OR graphs \cite{dechter2007and}, cutset networks \cite{rahman2014cutset}, and probabilistic sentential decision diagrams \cite{kisa2014probabilistic}  represent a class of \textit{tractable probabilistic models} which are often used in practice to compactly encode a large multi-dimensional joint probability distribution. Even though all of these models admit linear time computation of marginal probabilities (MAR task), only some of them \cite{NEURIPS2021_vergari,peharz2015foundations}, specifically those without any latent variables or having specific structural properties, e.g., cutset networks, selective SPNs, AND/OR graphs having small contexts, etc., admit tractable most probable explanation (MPE) inference\footnote{The MPE inference task is also called full maximum-a-posteriori (full MAP) inference in literature. In this paper, we adopt the convention of calling it MPE.}. 

However, none of these expressive PCs can efficiently solve the \textit{marginal maximum-a-posteriori (MMAP) task} \cite{peharz2015foundations,NEURIPS2021_vergari}, a task that combines MAR and MPE inference. 
%It is known to be an NP-hard problem even to approximate \cite{conatyApproximationComplexityMaximumPosterioriInferenceSumProduct}. %In face, it remains an NP-hard problem in these models just like in BNs and MNs. 
More specifically, the difference between MPE and MMAP is that given observations over a subset of variables (evidence), MPE finds the most-likely assignment to all other variables while MMAP finds the most-likely assignment to a subset of non-evidence variables while marginalizing over the rest. The MMAP problem has numerous real-world applications, especially in health care, natural language processing, computer vision, linkage analysis and diagnosis where hidden variables are present and need to be marginalized out \cite{bioucasdiasBayesianImageSegmentationusinghiddenfields2016, kiselevPOMDPPlanningMarginalMAPProbabilisticInferenceGenerative, leeApplyingMarginalMapSearchProbabilisticConformantb,NIPS2015_faacbcd5}. In terms of computational complexity, both MPE and MMAP are at least NP-hard in SPNs, a popular class of PCs \cite{peharz2015foundations,conaty17}. Moreover, it is also NP-hard to approximate MMAP in SPNs to $2^{n^\delta}$ fox fixed $0 \leq \delta < 1$,
where $n$ is the input size \cite{conaty17,mei2018maximum}. It is also known that the MMAP task is much harder than the MPE task and is NP-hard even on models such as cutset networks and AND/OR graphs that admit linear time MPE inference \cite{park&darwiche04,conaty17,decamposNewComplexityResultsMAPBayesianNetworks}. 

%It is known that the MMAP task is at least NP-hard in widely used PCs such as SPNs

To date, both exact and approximate methods have been proposed in literature for solving the MMAP tasks in PCs. Examples of exact methods include branch-and-bound search \cite{maua2020two, mei2018maximum}, transforming MMAP to integer linear programming (ILP) and then using an ILP solver for solving the latter \cite{maua2020two}, and circuit transformations via pruning \cite{choi2022solving}. These methods can be quite slow in practice and are not applicable when fast, real-time inference is desired. As a result, approximate approaches which require only a few passes over the PC are often used in practice. Approximate solutions can be obtained in several ways, e.g., converting the given MMAP task to an MPE task defined over both the query and unobserved variables, as done in SPNs and other mixture models \cite{poon2011sum}, or compiling the original model with unobserved variables to a model that is only defined over the observed variables and is tractable for MPE \cite{rahman2019look}. Although these approaches can provide fast answers at query time, they often yield MMAP solutions that are far from optimal. 


%Although these afoapproaches can provide fast answers at query time, they are often far from the true optimal and require an extra model transformation step. In this paper, we address the problem of improving the accuracy and efficiency of the MMAP task in PCs by using deep neural networks.


%Existing methods that try to exactly solve MMAP queries over PCs are based on branch-and-bound search \cite{maua2020two, mei2018maximum} or \verify{circuit transformations (pruning) \cite{choi2022solving}}. These methods are often impractical for answering these queries in real-time, and therefore approximate schemes are readily adopted. Approximate solutions can be obtained in several ways, e.g., converting the given MMAP task to an MPE task defined over both the query and unobserved variables, as done in SPNs and other mixture models \cite{poon2011sum}, or compiling the original model with unobserved variables to a model with observed variables only that is tractable for MPE \cite{rahman2019look}. Although these approaches can provide fast answers at query time, they are often far from the true optimal and require an extra model transformation step. In this paper, we address the problem of improving the accuracy and efficiency of the MMAP task in PCs by using deep neural networks.

%Deep neural networks have been used in the past to improve the representational power of PCs. For example, conditional PCs like conditional cutset networks \cite{rahman2019cutset, dong2022conditionally} and conditional sum-product-networks \cite{shao2020conditional} incorporate NNs in their structure to fit arbitrary complex conditional distributions. Their primary purpose is to act as discriminative classifiers and accurately predict conditional probabilities over random variables given evidence. This has led to a significant boost in the performance of PCs in representing tractable, expressive conditional distributions.  

In this paper, we propose to address the limitations of existing approximate methods for MMAP inference in PCs by using neural networks (NNs), leveraging recent work in the \emph{learning to optimize} literature \cite{li2016learning,fioretto_optimalpowerflows_2020,  donti_methodoptimizationhard_2020, zamzam_solutionsextremelyfast_2020, park_learningconstrainedoptimization_2023}.
In particular, several recent works have shown promising results in using NNs to solve both constrained and unconstrained optimization problems (see \citet{park_learningconstrainedoptimization_2023} and the references therein). 

The high level idea in these works is the following: given data, train NNs, either in a supervised or self-supervised manner and then use them at test time to predict high-quality, near-optimal solutions to future optimization problems in the domain of interest. A number of reasons have motivated this idea of \textit{learning to optimize} using NNs: 1) NNs are good at approximating complex functions (distributions), 2) once trained, they can be faster at answering  queries than search-based approaches, and 3) with ample data, NNs can learn accurate mappings of inputs to corresponding outputs. This has led researchers to employ NNs to approximately answer probabilistic inference queries such as MAR and MPE in Bayesian and Markov networks \cite{yoon2019inference, cui_variational_2022}\eat{that can be cast as optimization problems, for example, using variational inference techniques to compute MARs and MPEs in PGMs \cite{??}}. To the best of our knowledge, there is no prior work on solving MMAP in BNs, MNs, or PCs using NNs.  

This paper makes the following contributions. First, we propose to learn a neural network (NN) approximator for solving the MMAP task in PCs. Second, by leveraging the tractability of PCs, we devise a loss function whose gradient can be computed in time that scales linearly in the size of the PC, allowing fast gradient-based algorithms for learning NNs. Third, our method trains an NN in a self-supervised manner without having to rely on pre-computed solutions to arbitrary MMAP problems, thus circumventing the need to solve intractable MMAP problems in practice. Fourth, we demonstrate via a large scale experimental evaluation that our proposed NN approximators yield higher quality MMAP solutions as compared with existing approximate schemes.

%We make the following contributions in this paper: 1) we propose to learn a neural network approximator for solving the MMAP task in PCs, 2) leveraging the tractability of these expressive models, we devise a loss function that can efficiently be evaluated at each iteration of gradient descent, 3) our method trains an NN in a self-supervised manner without having to rely on pre-computed solutions to arbitrary MMAP problems, 4) empirical results on several state-of-the-art PCs show that neural approximators can significantly improve the accuracy of MMAP in PCs. 

    \eat{Note that, although the MPE task ($|Z| = 0$) is tractable in PCs without latent variables, for example cutset networks, it is an NP-hard problem in PCs with latent variables e.g. sum-product networks and many popular mixture models, that is, MPE becomes an MMAP task in PCs with latent variables and unfortunately inherits its computational complexities.
    \eat{The three most common inference tasks performed over PCs are: 1) computing the marginal probability (MAR) over a subset of random variables with or without evidence, 2) given evidence over a subset of variables, finding  the most-probable-explanation (MPE) or assignment to the rest of the variables, and 3) given evidence over a subset of variables, finding the maximum-a-posteriori (MMAP) assignment to some other subset of variables from the distribution that is consistent with the given evidence and obtained through marginalizing out the rest of the unobserved variables.} 

    
    }
   



==> content/2-prelim.tex <==
\section{Preliminaries}
\begin{figure*}
    \centering
    \resizebox{0.48\textwidth}{!}{\input{figures/pc1}}\quad
    \resizebox{0.48\textwidth}{!}{\input{figures/pc2}}
    \caption{Caption}
    \label{fig:example}
\end{figure*}
We denote random variables by uppercase letters, e.g. $X$ and there values by the respective lower case letters, e.g., $x$. Sets of random variables are denoted by bold upper case letters, e.g., $\mathbf{X}$, and their assignments by bold lower case letters, e.g., $\mathbf{x}$. We consider binary random variables taking values from $\{0, 1\}$. We use $\bar{X}$ to denote the complement of $X$. For any given integer $N$, we denote the set $\{1,\ldots,N\}$ by $[N]$.

\subsection{Probabilistic Circuits} PCs represent joint probability distributions using rooted directed acyclic graphs that consist the following three types of nodes.
\begin{itemize}
    \item Sum Nodes ($\oplus$): Sum nodes represent probabilistic conditioning over random variables in the domain (either observed or latent). Any edge $\langle m,n\rangle$ into a sum node $n$ from its child node $m$ is weighted by the (un)conditional probability $\omega(m,n)$  of the associated variable taking on a value in its domain. A normalized sum node has the following property: $\sum_{m\in ch(n)}\omega(m,n) = 1$, where $ch(n)$ is the set of children of node $n$. The distribution computed at a sum node $n$ is $P_n(\mathbf{x}) = \sum_{m\in ch(n)} \omega(m,n) P_m(\mathbf{x})$, where $P_m()$ is the distribution rooted by child node $m$.
    \item Product Nodes ($\otimes$): Product nodes represent the operation of decomposing a large problem into multiple, probabilistically independent sub-problems. The distribution computed at a product node $n$ is $P_n(\mathbf{x}) = \prod_{m\in ch(n)}P_m(\mathbf{x})$.
    \item Leaf Nodes: Leaf nodes represent simple functions (distributions) over observed variables in the domain. For example SPNs (\cite{poon2011sum}) and ACs (\cite{darwiche2003differential}) use indicators like $\mathbb{I}(X=1)$ and $\mathbb{I}(X=0)$\footnote{For brevity, We use $X$ to denote $\mathbb{I}(X=1)$ and $\bar{X}$ to denote $\mathbb{I}(X=0)$.} while cutset networks (\cite{rahman2014cutset}) have tree structured Bayesian networks at the leaves. 
\end{itemize}
Marginal probabilities are computed by evaluating the PC in a bottom-up manner by first evaluating the functions at the leaves and then propagating the values to the root performing sum-product operations along the structure. The complexity of such operations is thus bounded by the size of the circuit i.e. the total number of edges in its structure. 
\begin{figure}[htb]
    \centering
    \includegraphics[scale=1.25]{figures/pc.pdf}
    \vspace{-0.4cm}
    \caption{A PC representing a naive bayes mixture model over $\mathbf{E}=\{E_1,\ldots,E_m\}$ and $\mathbf{Q}=\{Q_1,\ldots,Q_n\}$. Solid edges from mixture (sum) nodes are weighted while dashed edges from product nodes are unweighted. To avoid clutter, we do not label the edges by their weights. The indicators for the query variables in $\mathbf{Q}$ are set according to the respective neural network outputs while the indicators for the evidence variables in $\mathbf{E}$ are set according to the given MMAP evidence. Both the indicators of any hidden variable are set to 1. } \label{fig:pc}
\end{figure}
\vspace{-0.30cm}
\begin{exmp}\label{exmp:pc}
    Figure \ref{fig:pc} shows an example PC representing a naive Bayes mixture model $P(\mathbf{E},\mathbf{Q},H)$ where $\mathbf{E}=\{E_1,\ldots,E_M\}$ and $\mathbf{Q} = \{Q_1,\ldots,Q_N\}$. The sum (mixture) node representing a \eat{latent}class variable $H$ at the root has $K$ components each weighted by $P(H=h_k)=\omega_k$ such that $\sum_{k\in[K]}\omega_{k} = 1$. Each component $k$ represents the joint distribution $P_k(\mathbf{E,Q}|H=h_k)=\prod_{m\in[M]}P_k(E_m)\prod_{n\in[N]}P_k(Q_n)$ using a subPC rooted by a product node having $(M+N)$ child sum nodes. Each of these sum nodes represents a Bernoulli distribution $P_k(.)$ as follows. The edges attached to the leaf indicators of a variable $E_m\in\mathbf{E}$ are weighted by $\alpha_{k,m}$ (left edges) and $(1 - \alpha_{k,m})$ (right edges). Similarly, edges attached to the leaf indicators of a variable $Q_n\in \mathbf{Q}$ are weighted by $\beta_{k,n}$ and $(1 - \beta_{k,n})$. The probability of a complete assignment $(h_k, \mathbf{e,q})$ is 
    \begin{align*}
        P(h_k,\mathbf{e,q}) & = P(h_k)\times P(\mathbf{e,q}|h_k)\\
        & = \omega_k\bigg(\prod_{m\in[M]}(\alpha_{k,m}e_m+(1-       \alpha_{k,m})(1 - e_m).\\
           &  \prod_{n\in[N]}(\beta_{k,n}q_n+(1-\beta_{k,n})(1-q_n))\bigg)
    \end{align*}
\end{exmp}  
\subsection{MMAP in Probabilistic Circuits}
The MMAP task is defined as follows. Given an assignment $\mathbf{e}$ to some subset of variables $\mathbf{E}$, we are interested in finding the most likely assignment \eat{$\mathbf{q}^*$} to another subset of variables $\mathbf{Q}$ by marginalizing out the rest of the variables in the subset $\mathbf{H}$. Mathematically, 
\eat{
\begin{align}
\label{eqn:mmap}
    \eat{\mathbf{q}^* & = }\argmax_{\mathbf{q}} P(\mathbf{e},\mathbf{q}) =\argmax_{\mathbf{q}} \sum_{\mathbf{h}} P(\mathbf{e, q, h})
\end{align}
}
The subsets $\mathbf{E, Q,}$ and $\mathbf{H}$ are respectively called the sets of \textit{evidence, query} and \textit{hidden} variables\footnote{We adopt the notations from \cite{choi2022solving}.}.Assuming $H$ is a latent class variable in example \ref{exmp:pc}, given evidence $\mathbf{E=e}$, the MMAP over the query variables $\mathbf{Q}$ can be found by solving the following multilinear program\footnote{\textcolor{red}{MMAP tasks can be formulated as integer linear programs (\cite{maua2020two}). We obtain linear programs by relaxing the integrality constraints.}}.
  \eat{  
    \begin{align*}  \argmax_{\mathbf{q}}\sum_{k\in[K]} \omega_k\bigg(\prod_{m\in[M]}(\alpha_{k,m}e_m+(1-\alpha_{k,m})(1 - e_m).\\
    \prod_{n\in[N]}(\beta_{k,n}q_n+(1-\beta_{k,n})(1-q_n)\bigg)
    \end{align*}
  }  



==> content/3-method.tex <==

\section{A Neural Optimizer for MMAP in PC\text{s}}\label{sec:method}
In this section, we introduce a machine learning approach that uses a neural network to predict answers to marginal MAP queries in PCs.  Formally, a \textit{neural network optimizer} for the MMAP task over a given PC is a deep neural network $f_\theta(.)$ parameterized by $\theta$ which takes as input an (possibly encoded) assignment $\mathbf{e}$ over the evidence variables and outputs an assignment $\hat{\mathbf{q}}$ over the query variables that is an optimal solution (in practice a close to optimal solution) to the MMAP problem defined in \ref{eqn:mmap}. For now, we will assume that the sets of evidence ($\mathbf{E} = \{E_i\}_1^N$), query ($\mathbf{Q}=\{Q_j\}_1^M$) and hidden ($\mathbf{H}=\{H_k\}_1^K$) variables are all fixed and known \textit{a priori} for each MMAP task posed to the PC. In the supplement, we propose a generalization to efficiently handle variable length, arbitrarily chosen evidence, query and hidden variables. Next, we describe how to train the parameters of $f_\theta(.)$ from data.

Given the architecture of $f_\theta(.)$, learning its parameters can be accomplished either in a supervised manner or in a self-supervised manner. In a supervised learning setting, data is given in the form $\mathcal{D} = \{\langle \mathbf{e}_1, \mathbf{q}_1^*,\ldots,\langle \mathbf{e}_n, \mathbf{q}_n^*\rangle\}$, where each input $\mathbf{e}_i$ is the evidence of an MMAP query and each output (label) $\mathbf{q}_i^*$ is its corresponding exact optimal solution according to the PC. At each iteration during training by gradient descent, the NN predicts an MMAP assignment $\hat{\mathbf{q}}_i = f_\theta(\mathbf{e}_i)$ for each input $\mathbf{e}_i\in\mathcal{D}$ according to its current set of parameters. It then back-propagates a supervised loss (error) like the mean-squared-error (MSE) $\frac{\sum_i(\mathbf{q}^*_i - \hat{\mathbf{q}}_i)^2}{n}$ or the mean-absolute-error (MAE) $\frac{\sum_i|\mathbf{q}^*_i - \hat{\mathbf{q}}_i|}{n}$ to update its parameters. This iterative minimization of the loss continues until convergence. Note that during such supervised training the PC under consideration is never queried. Although such supervised approaches allow us to use simple to implement loss functions, they require access to the exact solutions to several MMAP problems, potentially over high-dimensions, which are infeasible to obtain in practice\footnote{We do not propose the use of the training data to learn $f_\theta(.)$ in a supervised manner, since it is unlikely that the sampled $\mathbf{q}_i$'s in the dataset are optimal MMAP solutions to the sampled $\mathbf{e}_i$'s.}. \marginpar{TR:See footnote text} We therefore propose a self-supervised approach in the next section. 

\subsection{A Tractable Self-Supervised Loss}In a self-supervised learning setting, we are given data defined  over the input (evidence) variables only, i.e., $\mathcal{D} = \{\mathbf{e}_1,\ldots,\mathbf{e}_n\}$. We assume that each $\mathbf{e}_i \in \mathcal{D}$ has been sampled from the distribution $P(\mathbf{E}) = P(E_1)\prod_{i=2}^{N}P(E_i|E_{1:i-1})$. Each conditional distribution $P(E_i|E_{1:i-1})$ can be computed exactly by performing tractable marginal inference over the given PC. At any given iteration, the NN predicts an MMAP assignment $\hat{\mathbf{q}}_i = f_\theta(\mathbf{e}_i)$. We define a loss $\ell_i(\mathbf{e}_i, \hat{\mathbf{q}}_i)$ for each predicted assignment as the unnormalized negative (log) probability $-P(\mathbf{e}_i, \hat{\mathbf{q}}_i)$ according to the given PC. The total loss $\mathcal{L}(.)$ to be minimized can therefore be defined as the average of these individual losses. Mathematically, 
\begin{align}\label{eqn:loss}
    \mathcal{L}(\mathcal{D}) & = \frac{1}{n}\sum_{i=1}^n\ell_i(\mathbf{e}_i, \hat{\mathbf{q}}_i) =  \frac{1}{n}\sum_i^n-P(\mathbf{e}_i, \hat{\mathbf{q}}_i)\nonumber\\
    & = -\frac{1}{n}\sum_{i=1}^n\bigg(\sum_\mathbf{h}P(\mathbf{e}_i,\hat{\mathbf{q}}_i,\mathbf{h})\bigg) 
\end{align}
Since each predicted assignment $\hat{\mathbf{q}}_i = \{\hat{q}_{1,i},\ldots,\hat{q}_{M,i}\}$ is a continuous vector in $[0,1]^M$, loss $\ell(\mathbf{e}_i, \hat{\mathbf{q}}_i)$ is a linear approximation to the ILP formulation of the MMAP problem given by $\mathbf{e}_i$. Finally, computing the gradients $\frac{\partial\mathcal{L}}{\partial\hat{\mathbf{q}}_i}$'s can be done efficiently since loss $\mathcal{L}(.)$ is tractable; each $\ell_i(.)$ is bounded by the size of the PC. 

\subsubsection{On Finding Discrete Solutions}
\label{sec:entropy}
One approach to obtain discrete MMAP solutions is to round each continuous output $\hat{q}_i\in[0,1]$ to the nearest integer. This approach may result in inaccurate sub-optimal solutions. We propose to add the following penalty to the loss $\mathcal{L}(.)$ that encourages discrete solutions by minimizing the sum of the entropies over the output variables.
\begin{equation*}
    \mathcal{L}(\mathcal{D}) - \alpha \sum_{j=1}^n\sum_{i=1}^M\bigg(\hat{q}_{i,j}\log(\hat{q}_{i,j}) + (1-\hat{q}_{i,j})\log(1-\hat{q}_{i,j})\bigg)
\end{equation*}
where $\alpha$ is a hyperparameter and each $\hat{q}_{i,j}$ is the predicted quantity $\hat{P}(Q_i = 1|\mathbf{e}_j)$ ($i^{th}$ output) on the $j^{th}$ input. 

\sva{Need to add a subsubsection for case where we also train on the test set}



==> content/4-experiments.tex <==

\section{Experiments}
In this section, we conduct a comprehensive evaluation to assess the effectiveness of our novel \textit{self-supervised} MMAP solver, referred to as \our hereafter. The evaluation focuses on a range of diverse inference tasks, demonstrating the versatility and capabilities of our proposed solution. To establish a comprehensive comparison, we contrast \our with a variety of MMAP inference approaches within probabilistic circuits (PCs). We proceed to assess these competing methods across several test problems, utilizing two key criteria for evaluation: log likelihood scores and inference times.




\eat{For this initial study we chose the NN architecture to be ...Table}


\subsection{Competing Methods}
\label{sec:exp-methods}
In the initial phase, we undertake a comparative analysis between our \our method and three baseline MMAP inference methods: \spn, Maximum Likelihood approximation, and Sequential Approximation. These methods are then employed as initialization techniques for the subsequent local search procedure (\spnls, \mlels, \seqls, and \ourls). Each of these methods approximates the query variables within the MMAP task. We aim to assess the performance of these initialization strategies and subsequently examine their efficacy when integrated into the local search algorithm.

\subsubsection{\spn}
The MMAP state is derived by substituting sums with maximizations. During the upward pass, a max node produces the maximum weighted value from its children instead of their weighted sum. Subsequently, the downward pass begins from the root and iteratively selects the highest-valued child of a max node (or one of them), along with all children of a product node. As per \cite{poon2011sum}, this approach is demonstrated to locate the state, provided that the Sum-Product Network (SPN) is consistent.

\subsubsection{Maximum Likelihood Approximation (\mle)}
For every MAP variable Q, we assign its value to the instance q that maximizes the probability $P(q | e)$. 

\subsubsection{Sequential Approximation (\seq)}
This method takes into account the MAP variables $Q_1, Q_2, \ldots, Q_m$, selecting at each step a variable $Q_i$ that maximizes the probability $P(q_i | e, y)$ for one of its values $q_i$, where $y$ represents the instantiation of previously considered MAP variables.

\subsection{Stochastic Hill Climbing Search}
Stochastic hill climbing is an iterative optimization technique that entails making incremental adjustments to either a variable's state, with the goal of achieving the maximum change in probability, or selecting a variable at random for modification. In our experiments, we harness the \our method, alongside the aforementioned techniques, as the initial starting points for the hill climbing process. Through an analysis of the scores obtained from these diverse initializations, we gain insights into which method serves as the more effective initialization for the hill climbing procedure. This evaluation provides us with insights into the relative performance of these methods when employed as initialization strategies. Throughout the experiments, we conducted a search for 100 iterations.

\subsection{Models}
\subsubsection{Probabilistic Circuits}
For learning the structure and parameters of the probabilistic circuits (PCs), we utilized the DeeProb-kit library \cite{loconte2022deeprob}. The sizes of the probabilistic circuits (PCs) vary, encompassing a range from 46 to 22027.  
\eat{with randomly chosen 60\% of the variables as evidence (input) and 40\% of the variables as query (output).}
We employed a systematic approach to determine the number of query variables as a fraction of the total variables, denoted as $query ratio \times |variables|$. \eat{Further details are provided in sections \ref{subsec:exp_binarydataset, subsec:exp_imagecompletion}}



\subsubsection{Neural Optimizers}
For each dataset, a corresponding neural network was trained to minimize the loss function in \ref{eqn:loss}. Neural network inputs are determined by the size of the encoding of evidence variables, and outputs are based on the number of query variables. Each neural network consists of four layers, with the number of nodes in the $i^{th}$ layer calculated using $128 \times (2^i)$. The neural networks underwent 50 epochs using the Adam optimizer \citep{Kingma2014Dec} with a learning rate of $1 \times 10^{-3}$. A Learning Rate Scheduler was implemented to adaptively modify the learning rate by decaying it for each parameter group by a factor of gamma after a pre-defined number of epochs. The models' training and testing processes were carried out on a single NVIDIA A40 GPU.

\subsection{Enhancing Fast and Accurate MMAP Query Resolution for PCs}
\label{subsec:exp_binarydataset}



% \input{content/tables/contingency_mpe-search}
% \input{content/tables/contingency_mmap-search}

Our initial series of experiments centers around a collection of twenty-two widely recognized benchmark datasets commonly utilized for training tractable probabilistic models. \eat{This comprehensive dataset collection includes NLTCS, MSNBC, KDDCup2k, Plants, Audio, Jester, Netflix, Book, EachMovie, WebKB, Reuters-52, and 20 NewsGroup} \cite{lowdLearningMarkovNetwork2010b}, \eat{as well as Accidents, Retail, Pumsb-star, DNA, Kosarek, and BBC datasets} \cite{haarenMarkovNetworkStructureLearningRandomizedFeature2012}, \eat{. Additionally, we incorporated datasets such as Mushrooms, Connect 4, RCV-1} \cite{larochelleNeuralAutoregressiveDistributionEstimator},\eat{ and Movie reviews} \cite{bekkerTractableLearningComplexProbabilityQueries}. These datasets were chosen to facilitate the learning of sum-product networks (SPNs), a versatile probabilistic model known for its success across diverse application domains. Across this array of datasets, we observed a diverse range of variable counts, with the minimum comprising 16 variables and the maximum extending to 1058. 

We generated marginal MAP instances for two distinct scenarios: one where none of the variables from the dataset are included in set $H$, and another where dataset variables are incorporated in $H$. Specifically, we explored a range of $query ratio$ values for the binary datasets, namely $\{0.9, 0.8, 0.7, 0.6, 0.5, 0.3, 0.1\}$. This meticulous approach allowed us to examine varying proportions of evidence variables across the datasets thoroughly. In the situation where $H$ also contains the dataset variables, we further segregated the variables in the evidence set into two buckets: one assigned to $E$ and the other allocated to $H$. Our analysis involved a comprehensive range of experiments. With 22 diverse datasets and the consideration of 7 potential values for the $query ratio$ parameter, we conducted a total of 154 experiments for each of the previous scenarios. This cumulative effort amounted to a  total of 308 experiments.

\input{content/tables/contingency-base}

In this sequence of experiments, we initiate by providing contingency tables that encompass both our proposed \our method and the methodologies described in Section \ref{sec:exp-methods}. These outcomes are detailed in Table \ref{tab:contingency-base}. In this table, the value located at the $i^{th}$ row and $j^{th}$ column signifies the instances where the $i^{th}$ method exhibited superior performance to the $j^{th}$ method. Therefore, higher values within a row indicate that the corresponding method outperformed the competing methods. 
The subset of experiments that remain is obtained by subtracting the combined values from the $i^{th}$ row and $j^{th}$ column, as well as the $j^{th}$ row and $i^{th}$ column, from the total count of experiments. This subset reflects instances in which the mean log likelihood scores exhibited equality between the two compared methods. 
\eat{We also present the results for the method where we incorporate entropy as a penalty, as introduced in Section \ref{sec:entropy}, referred to as \ourentropy and method that .} 
We also conduct a comparative analysis between the \our method and \spn to assess how well the \our method performs compared to the commonly used baseline for SPN inference. In the heat-map representation, the y-axis represents the datasets (ordered by ascending number of variables), while the x-axis signifies the query ratio. The values in the bin represent the percentage difference between the Mean Log Likelihood scores of \our method and \spn method. The formula is given in Equation \ref{eq:percent_diff}

\begin{equation}
\label{eq:percent_diff}
\begin{aligned}
\% \text{Diff.} = \frac{(\text{\ourfig LL Mean} - \text{\spn LL Mean}) \times 100}{|\text{\spn LL Mean}|}
\end{aligned}
\end{equation}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{content/figures/mpe_nn_spn_heatmap.pdf}
        \caption{\mpe}
        \label{fig:mpe_nn_vs_spn}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{content/figures/mmap_nn_spn_heatmap.pdf}
        \caption{\mmap}
        \label{fig:mmap_nn_vs_spn}
    \end{subfigure}
    
    \caption{Heat map showing the percentage difference in log-likelihood scores between \texttt{OurMethod} and \texttt{SPN}. Blue color represents \texttt{SPN}'s superiority (negative values), while red color represents \texttt{OurMethod}'s superiority (positive values).}
    \label{fig:performance_vs_spn}
\end{figure}

Let's begin by examining the scenario where none of the variables from the dataset are included in $H$. The results of this particular experiment set are outlined on the left side Table \ref{tab:contingency-base} titled \mpe. Remarkably, the \our method exhibits superior performance compared to the other baseline methods in more than half of the experiments. This outcome underscores the efficacy of the neural network in addressing \mpe queries across varying levels of complexity. 
\eat{Furthermore, we present the outcomes for the method referred to as \ourtt, where training is conducted on the test set. Remarkably, this approach surpasses the performance of the \our method, outperforming it in 50 instances. Notably, \ourtt even exhibits superior performance compared to the baseline methods in more cases than the \our method. This observation underscores the notion that allowing the neural network to learn the distribution of the test set for a brief duration can yield even better results. The entropy-based method, referred to as \ourentropy, also demonstrates superior performance compared to the other baseline techniques in nearly half of the instances.} 
Additionally, the corresponding heatmaps are illustrated in Figure \ref{fig:mpe_nn_vs_spn}. Upon observation, it becomes apparent that the \our method competes closely with \spn when the size of the query set is small. However, as the number of query variables increases, signaling a more challenging problem, the \our method consistently outperforms or maintains parity with the \spn method across all datasets, except for accidents, pumsb-star, and book.

Subsequently, we explore the case where specific variables from the dataset can also be included in $H$. Notably, due to the encoding method used for inputs, the values of these nodes remain unutilized by the neural network. The complexity of the problem increases as the neural optimizer receives less information. The results of these experiments are depicted on the right side of Table \ref{tab:contingency-base} titled \mmap. Despite the elevated complexity of this experiment set, the performance of the neural approximator further improves. The neural approximator outperforms the \spn and \mle methods in almost two-thirds of the experiments and the \seq method in half of the experiments. This pattern underscores the neural approximator's ability to enhance its performance as the task complexity increases. 
\eat{The \ourtt and \ourentropy methods continue to exhibit exceptional performance in this scenario, surpassing the \our method in 51 and 65 instances, respectively. They once again build upon the advancements achieved by the \our method across all the other baselines, aligning with the previously observed trend. Despite incurring minimal overhead, these methods offer substantial enhancements, underscoring that their consistently positive outcomes warrant further exploration and consideration.}
Figure \ref{fig:mmap_nn_vs_spn} shows the corresponding heatmaps for this scenario. A similar trend is evident in these experiments when the query ratio is higher. Notably, the \our method consistently delivers superior performance, even with fewer query variables. This underscores how the \our method excels in handling more challenging problems, even as the performance of the \spn method diminishes. Comprehensive information encompassing means and standard deviations of log-likelihood scores for each experimental set is provided in the supplementary section. 

\input{content/tables/contingency-hill-climbing}

We also investigate the effectiveness of \our method and other baseline approaches when employed as initialization strategies for Hill Climbing Search. These findings are illustrated in Table \ref{tab:contingency-hill}. The results for \mpe are presented on the left side, while those for \mmap are presented on the right. Notably, \our method showcases exceptional performance as an initialization technique for both \mpe and \mmap tasks. Specifically, it outperforms all other baseline approaches in nearly two-thirds of the experiments. This indicates that our method not only excels on its own but can also serve as a valuable initialization technique for enhancing the outcomes of hill climbing searches.
% In Figures \ref{fig:mpe_vs_query_ratio} and \ref{fig:mmap_vs_query_ratio}, we additionally illustrate the count of datasets where the \our method outperforms the \spn method in relation to the query ratio. As the task complexity escalates (with a higher query ratio), the frequency of \our outperforming \spn also rises.
\sva{
\textbf{Can also include times for MPE - can select one of the following paragraphs. The first paragraph shows time for MMAP queries while the second paragraph shows time for both MPE and MMAP.}}

\sva{On average, the \our method proves to be the swiftest, requiring only 7.45 microseconds ($\mu$s) to solve an MMAP query. This showcases its remarkable efficiency compared to the \spn method, which has an average inference time of 6660.41 $\mu$s, making the \our method approximately 893.75 times faster. Additionally, the \our method demonstrates its rapidity by being around 58151.78 times faster than \mle, with an average inference time of 433358.17 $\mu$s, and a remarkable 85746.29 times faster than \seq, with an average query time of 638997.73 $\mu$s. }

\sva{On average, the \our method demonstrates remarkable speed, solving an MMAP query in just $7.45 \, \mu$s and an MPE query in $8.89 \, \mu$s. We present the speedup ratios and timings in the format "MMAP (MPE)" for subsequent methods. This efficiency shines in comparison to the \spn method, which requires an average inference time of $6.66041 \times 10^3$ ($1.274881 \times 10^4$) $\mu$s, making our \our method approximately $8.9375 \times 10^2$ ($1.43552 \times 10^3$) times faster. Moreover, our approach showcases its agility by surpassing the \mle method by approximately $5.815178 \times 10^4$ ($7.710485 \times 10^4$) times, with an average inference time of $4.3335817 \times 10^5$ ($6.84767 \times 10^5$) $\mu$s, and demonstrating a remarkable $8.574629 \times 10^4$ ($1.15797 \times 10^5$) times speedup over the \seq method, with an average query time of $6.3899773 \times 10^5$ ($1.028392 \times 10^6$) $\mu$s.}

Further elaboration on the running times can be found in the supplementary section.

Leveraging the full computational potential of GPU processing, the \our method enables queries to be resolved in real-time, contributing to its exceptional performance. Additional information regarding the inference times for all the methods will be elaborated upon in the supplementary section. This detailed analysis will offer a comprehensive understanding of the time taken by each method to perform inferences, providing a more thorough insight into their respective efficiencies and performance characteristics.

\input{content/tables/contingency-cifar-base}

To assess the method's performance across additional real-world datasets, we embarked on experiments employing the Binarized CIFAR dataset \cite{krizhevskyLearningMultipleLayersFeaturesTinyImages}. We selected nine distinct classes, with each image initially encoded as a binary vector. Subsequently, we trained sum-product networks (SPNs) on these encoded representations. Our findings, as depicted in Table \ref{tab:cifar10-base}, consistently reveal the NN method's supremacy across all classes. This compellingly demonstrates the \our method's adeptness in surpassing alternative methodologies in real-world scenarios. Given its commendable performance and efficient execution time, \our method emerges as a robust candidate for diverse query computations on PCs.


\subsection{Efficient Image Completion with Limited Data: MNIST and EMNIST Analysis}
\label{subsec:exp_imagecompletion}
Furthermore, we delved into the task of image completion using the Binarized MNIST dataset \cite{salakhutdinov2008quantitative} and the Binarized EMNIST dataset \cite{cohenEMNISTExtensionMNISThandwrittenletters2017}. In this context, we specifically selected $query ratio$ value of $\{0.7\}$ to drive this series of experiments. We utilized the top portion of the image as evidence, leaving the bottom portion to be completed. 
% \input{content/tables/contingency_mnist-base}
% \vspace*{-5pt}
% \input{content/tables/contingency_emnist-base}
\input{content/tables/contingency-mnist-emnist-base}
Once again, we employ contingency tables to gain insights into the performance of various methods. Let's begin by examining the contingency table for the MNIST and EMNIST datasets, as depicted in Table \ref{tab:mnist-base}. In the context of the ten classes within the MNIST dataset, the \our method outperformed all other baseline methods in nine instances. Shifting our focus to the EMNIST dataset, detailed results are presented on the right side of the table. Within this dataset, featuring eight selected classes, the \our method exhibited superior performance compared to all other baselines in seven cases. This demonstration underscores the applicability of the \our method in real-world scenarios, such as image completions, where it excels by offering enhanced performance and expedited results compared to other inference techniques employed in probabilistic contexts. In consideration of space limitations, we present qualitative results for the MNIST and EMNIST datasets in the supplementary section.

\subsection{Summary}

\eat{For both datasets, the \ourtt method outperforms the \our method in 9 out of 10 cases and 3 out of 8 cases, respectively. Similarly, the \ourentropy method outperforms the \our method three times for both datasets, showcasing consistent trends across the experiments.}

\eat{
% Qualitative Results for MNIST and EMNIST
\begin{figure}[h]
    \centering
    \setlength{\tabcolsep}{10pt} % Adjust spacing between subfigures
    
    \begin{tabular}{@{}cc@{}}
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/mnist_5_623.png}
            \caption{MNIST Digit 5}
        \end{subfigure} &
        
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/mnist_6_589.png}
            \caption{MNIST Digit 6}
        \end{subfigure} \\
        
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/mnist_8_38.png}
            \caption{MNIST Digit 8}
        \end{subfigure} &
        
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/mnist_9_422.png}
            \caption{MNIST Digit 9}
        \end{subfigure} \\
    \end{tabular}
    
    \vspace{1em} % Add vertical spacing for visual balance
    
    \begin{tabular}{@{}cc@{}}
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/emnist_1_420.png}
            \caption{EMNIST Character A}
        \end{subfigure} &
        
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/emnist_3_526.png}
            \caption{EMNIST Character C}
        \end{subfigure} \\
        
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/emnist_19_388.png}
            \caption{EMNIST Character S}
        \end{subfigure} &
        
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/emnist_22_763.png}
            \caption{EMNIST Character V}
        \end{subfigure} \\
    \end{tabular}
    
    \caption{Image Completions for MNIST and EMNIST datasets. First image: Original. Second image: \spn Completion. Third image: \our Completion. The gray line separates evidence (above) from query (below).}
    \label{fig:image-completion}
\end{figure}

Qualitative image completions for MNIST and EMNIST datasets are presented in Figure \ref{fig:image-completion}. Beginning with the original image as the initial reference, followed by the \spn method's completion attempt, and culminating in our novel \our method's completion. Specifically, characters such as 8, 9, A, and S exhibit discontinuities in their \spn-generated completions, as the lower portions fail to align with their upper counterparts seamlessly. This showcases the arduous nature of the challenge and underscores the limitations of the \spn method in handling such intricate tasks. In stark contrast, the proposed \our method offers a remarkable improvement in completion quality. It adeptly addresses the difficulties posed by limited available information and generates reconstructions that are not only smoother but also exhibit a remarkable coherence. This highlights \our method's efficacy in real-world scenarios with limited information but extensive query needs.}

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{content/figures/nist/mnist.pdf}
%         \caption{MNIST -ve Log Likelihood Scores}
%         \label{fig:mpe_nn_vs_spn}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{content/figures/nist/emnist.pdf}
%         \caption{EMNIST -ve Log Likelihood Scores}
%         \label{fig:mmap_nn_vs_spn}
%     \end{subfigure}
    
%     \caption{Performance Comparison}
%     \label{fig:performance_vs_spn}
% \end{figure}

\eat{
\subsection{Training}
To ensure that the NN performs at least as good as the PC on approximating MMAP, we perform a pretraining step.
\subsection{Results}

A fast approximate method to solve \ref{eqn:mmap} is to replace the inner summation by a maximization over $\mathbf{h}$. This is equivalent to switching sum nodes to max nodes in a PC and then performing a bottom pass followed by a top-down pass to construct an assignment $\langle \mathbf{q}^*,\mathbf{h}^*\rangle$. The MMAP solution is then approximated by the partial assignment $\mathbf{q}^*$, ignoring $\mathbf{h}^*$.
\subsubsection{To Discuss}
\begin{itemize}
    \item Overfitting? MMAP value of NN $>$ MMAP value of SPN on training data, but the opposite relation holds in most of the test samples. 
    \item What kind of regularizations can we use? 
\end{itemize}
}

==> content/5-conclusion.tex <==
\section{Conclusion and Future Work}
\eat{In this paper we presented a machine learning based method to solve the MMAP task over PCs. 
\textbf{Neural Approximators for MPE over intractable models}}
In this paper, we introduced a novel self-supervised learning algorithm for solving MMAP and MPE queries in PCs. Our contributions comprise a neural network approximator and a self-supervised loss function which leverage the tractability of PCs for achieving scalability. Notably, our method employs minimal hyperparameters, requiring only one in the discrete case. We conducted a comprehensive empirical evaluation across various benchmarks; specifically, we experimented with 22 binary datasets used in tractable probabilistic models community and three classic image datasets, MNIST, EMNIST, and CIFAR-10. We compared our proposed neural approximator to polytime baseline techniques and observed that it is superior to the baseline methods in terms of log-likelihood scores and is significantly better in terms of computational efficiency. Additionally, we evaluated how our approach performs as an initialization scheme in stochastic hill climbing (local) search and found that it improves the quality of solutions output by anytime local search schemes. Our empirical results clearly demonstrated the efficacy of our approach in both accuracy and speed. 

Future work includes compiling PCs to neural networks for answering more complex queries that involve constrained optimization; developing more accurate self-supervised loss functions; learning better NN architecture for the given PC; etc.

%In considering the limitations inherent in our proposed method, we recognize the potential for future work to address these challenges. Our approach currently lacks applicability in cases involving random queries, evidence, and unobserved variables, prompting the exploration of strategies to extend its scope to encompass such scenarios. Additionally, given the method's reliance on the quality of the underlying Probabilistic Circuit (PC), mitigating susceptibility to poorly trained PCs becomes a key avenue for future investigation. Furthermore, the requirement for ample training data to achieve accurate self-supervised learning representations, particularly in domains with limited data availability like the Olivetti faces dataset, calls for the exploration of innovative techniques to enhance performance and prevent overfitting. 

==> content/algo.tex <==
\begin{algorithm}\label{algo:a1}
\caption{A Neural Network Optimizing MMAP(\texttt{SS-CMPE})} %($\mathcal{D}, \mathcal{F}_\theta, f, g, \epsilon$)}
\begin{algorithmic}[1]
%\Function{Train}{$NN, X, F, G, eps$}
%\Require{Where \\ $NN$ = Randomly Initialized Auto Encoder, \\
\Require{$\mathcal{F}_\theta$ := A Neural Network with randomly initialized parameters $\theta$, $\mathcal{D}$ := $\{\mathbf{x}_i\}_1^N$, $\mathcal{P}$ := A PC} %$G$ = Constraint g, \\
%$\epsilon$ := weight to add to the factor,
%$\beta$:=Hyper-parameter}
%\Ensure{$NN$ (Trained NN which outputs a solution that satisfies constraints and optimizes the objective function when a X is given)}
\Ensure{$\mathcal{F}_\theta$ trained on $\mathcal{D}$ to minimize loss in \ref{eqn:loss_1}}
\For{$t = 1$ to $T$}
\Comment{T:=Maximum number of iterations}
\State $\{\hat{\mathbf{y}_i}\}_1^N =  \mathcal{P}(\{mathbf{x}_i\}_1^N)$
%\State $g_y =  G(y_{pred})$
%\State $mask = (g_y > 0)$ \Comment{$g_y$ is a vector, If %$g_y^{(i)}<0$, $mask^{(i)} = +1$, else $mask^{(i)}=-1$}
\State $\mathcal{L} = 0$ 
\Comment{Loss function}
\For{$i = 1$ to $N$}
\If {$g(\mathbf{x}_i, \hat{\mathbf{y}}_i) < 0$}
\State $\mathcal{L} = \mathcal{L} + f(\mathbf{x}_i, \hat{\mathbf{y}}_i)$ \Comment{Constraint is satisfied} %\Comment{$loss\_satisfied = F(y_{pred})$}
\Else
\State $\mathcal{L} = \mathcal{L} + \alpha_{\mathbf{x}_i} \times (f(\mathbf{x}_i, \hat{\mathbf{y}}_i) + g(\mathbf{x}_i, \hat{\mathbf{y}}_i))$ \Comment{Constraint is violated}
% Add section here
\EndIf
\EndFor
\State Back-propagate the $\mathcal{L}$

\EndFor
%\EndFunction
\end{algorithmic}
\end{algorithm}


==> content/experiments-vibhav.tex <==

\section{Experiments}
In this section, we describe and analyze the results of our comprehensive experimental evaluation for assessing the performance of our novel \underline{S}elf-\underline{S}upervised learning based \underline{M}MAP solver for \underline{P}Cs, referred to as \our hereafter. We begin by describing our experimental setup including competing methods, evaluation criteria, as well as NN architectures, datasets, and PCs used in our study.


%and analyze results a comprehensive evaluation to assess the effectiveness of our novel \textit{self-supervised} MMAP solver, referred to as \our hereafter. The evaluation focuses on a range of diverse inference tasks, demonstrating the versatility and capabilities of our proposed solution. To establish a comprehensive comparison, we contrast \our with a variety of MMAP inference approaches within probabilistic circuits (PCs). We proceed to assess these competing methods across several test problems, utilizing two key criteria for evaluation: log likelihood scores and inference times.




\eat{For this initial study we chose the NN architecture to be ...Table}


\subsection{Competing Methods}
\label{sec:exp-methods}
We used \textit{three polytime baseline methods} from the PC and probabilistic graphical models literature \cite{park&darwiche04,poon2011sum}. We also compared the impact of using the solutions computed by the three baseline schemes as well our method \our as initial state for stochastic hill climbing search.

%In the initial phase, we undertake a comparative analysis between our \our method and three baseline MMAP inference methods: \spn, Maximum Likelihood approximation, and Sequential Approximation. These methods are then employed as initialization techniques for the subsequent local search procedure (\spnls, \mlels, \seqls, and \ourls). Each of these methods approximates the query variables within the MMAP task. We aim to assess the performance of these initialization strategies and subsequently examine their efficacy when integrated into the local search algorithm.

\noindent\textbf{Baseline 1: MAX Approximation (\spn)}. In this scheme \cite{poon2011sum}, the MMAP assignment is derived by substituting sum nodes with max nodes. During the upward pass, a max node produces the maximum weighted value from its children instead of their weighted sum. Subsequently, the downward pass begins from the root and iteratively selects the highest-valued child of a max node (or one of them), along with all children of a product node. %As per , this approach is demonstrated to locate the state, provided that the Sum-Product Network (SPN) is consistent.

\noindent\textbf{Baseline 2: Maximum Likelihood Approximation (\mle)} \cite{park&darwiche04}
For each variable $Q \in \mathbf{Q}$, we first compute the marginal distribution $\text{p}_\mathcal{M}(Q|\mathbf{e})$ and then set $Q$ to $\argmax_{j \in \{0,1\}}\text{p}_\mathcal{M}(Q=j|\mathbf{e})$.% (namely assignment that maximizes $\text{p}_\mathcal{M}(Q|\mathbf{e})$).%  
%select value to the instance q that maximizes the probability $P(q | e)$. 

\noindent\textbf{Baseline 3: Sequential Approximation (\seq)}
In this scheme \cite{park&darwiche04}, we assign the query variables one by one until no query variables remain unassigned. At each step, we choose an unassigned query variable $Q_j \in \mathbf{Q}$ that maximizes the probability $\text{p}_\mathcal{M}(q_j|\mathbf{e},\mathbf{y})$ for one of its values $q_j$ and assign it to $q_j$ where $\mathbf{y}$ represents the assignment to the previously considered query variables.

%we select an arbitrary order over the query variables, say $(Q_1,\ldots,Q_M)$, and then m
%This method takes into account the MAP variables $Q_1, Q_2, \ldots, Q_m$, selecting at each step a variable $Q_i$ that maximizes the probability $P(q_i | e, y)$ for one of its values $q_i$, where $y$ represents the instantiation of previously considered MAP variables.

\noindent\textbf{Stochastic Hill Climbing Search.} We used the three baselines and our \our method as the initial state in stochastic hill climbing search for MMAP inference described in \cite{park&darwiche04}. The primary goal of this experiment is to assess whether our scheme can assist local search-based \textit{anytime methods} in reaching better solutions than other heuristic methods for initialization. In our experiments, we ran stochastic hill climbing for 100 iterations for each MMAP problem.

\subsection{Evaluation Criteria}
We evaluated the performance of the competing schemes along two dimensions: log-likelihood scores and inference times. Given evidence $\mathbf{e}$ and query answer $\mathbf{q}$, the log-likelihood score is given by $\ln \text{p}_\mathcal{M}(\mathbf{e},\mathbf{q})$.

%Stochastic hill climbing is an iterative optimization technique that entails making incremental adjustments to either a variable's state, with the goal of achieving the maximum change in probability, or selecting a variable at random for modification. In our experiments, we harness the \our method, alongside the aforementioned techniques, as the initial starting points for the hill climbing process. Through an analysis of the scores obtained from these diverse initializations, we gain insights into which method serves as the more effective initialization for the hill climbing procedure. This evaluation provides us with insights into the relative performance of these methods when employed as initialization strategies. Throughout the experiments, we conducted a search for 100 iterations.

%\subsection{Models}
\subsection{Datasets and Probabilistic Circuits}
We used twenty-two widely used binary datasets from the tractable probabilistic models literature \cite{lowdLearningMarkovNetwork2010b,haarenMarkovNetworkStructureLearningRandomizedFeature2012,larochelleNeuralAutoregressiveDistributionEstimator,bekkerTractableLearningComplexProbabilityQueries} (we call them TPM datasets) as well as the binarized MNIST \cite{salakhutdinov2008quantitative}, EMNIST \cite{cohenEMNISTExtensionMNISThandwrittenletters2017} and CIFAR-10 datasets.   
We used the DeeProb-kit library \cite{loconte2022deeprob} to learn a PC for each dataset. The number of nodes in these learned PCs ranges from 46 to 22027.

For each PC and each test example in the 22 TPM datasets, we generated two types of MMAP instances: MPE instances in which $\mathbf{H}$ is empty and MMAP instances in which $\mathbf{H}$ is not empty. We define query ratio, denoted by $qr$, as the fraction of variables that are part of the query set. We used the following values for $qr$: $\{0.1,0.3,0.5,0.6,0.7,0.8,0.9\}$. For generating MMAP instances, we used 50\% of the remaining variables as evidence variables (and for MPE instances all remaining variables are evidence variables). 

For the MNIST, EMNIST, and CIFAR-10 datasets, we used $qr=0.7$ and generated MPE instances only. More specifically, we used the top 30\% portion of the image as evidence, leaving the bottom 70\% portion as query variables. Also, in order to reduce the training time for PCs, note that for these datasets, we learned a PC for each class, yielding a total of ten PCs for each dataset.


\eat{with randomly chosen 60\% of the variables as evidence (input) and 40\% of the variables as query (output).}
%We employed a systematic approach to determine the number of query variables as a fraction of the total variables, denoted as $query ratio \times |variables|$. \eat{Further details are provided in sections \ref{subsec:exp_binarydataset, subsec:exp_imagecompletion}}



\subsection{Neural Network Optimizers}
For each PC and query ratio combination, we trained a corresponding neural network (NN) using the loss function described in the previous section. Because we have 22 TPM datasets and 7 query ratios for them, we trained 154 NNs for the MPE task and 154 for the MMAP task. For the CIFAR-10, MNIST and EMNIST datasets, we trained 10 NNs, one for each PC (recall that we learned a PC for each class).

Because our learning method does not depend on the specific choice of neural network architectures, we use a fixed neural network architecture across all experiments: fully connected with four
hidden layers having 128, 256, 512, and 1024 nodes respectively. We used ReLU activation in the hidden layers, sigmoid in the output layer, dropout for regularization \cite{srivastava_waypreventneural_2014} and Adam optimizer \cite{kingma_stochasticoptimization_2017} with a standard learning rate scheduler for 50 epochs. All NNs were trained using PyTorch \cite{paszke2019pytorch} on a single NVIDIA A40 GPU. We select a value for the hyperparameter $\alpha$  used in our loss function (see equation \eqref{eqn:loss}) via 5-fold cross validation. 

%leNeural network inputs are determined by the size of the encoding of evidence variables, and outputs are based on the number of query variables. Each neural network consists of four layers, with the number of nodes in the $i^{th}$ layer calculated using $128 \times (2^i)$. The neural networks underwent 50 epochs using the Adam optimizer \citep{Kingma2014Dec} with a learning rate of $1 \times 10^{-3}$. A Learning Rate Scheduler was implemented to adaptively modify the learning rate by decaying it for each parameter group by a factor of gamma after a pre-defined number of epochs. The models' training and testing processes were carried out on a single NVIDIA A40 GPU.

\subsection{Results on the TPM datasets}
\input{content/tables/contingency-base}
We summarize our results for the competing schemes (3 baselines and \our) on the 22 TPM datasets using the two contingency tables given in Table \ref{tab:contingency-base}, one for MPE and one for MMAP. Detailed results are provided in the supplementary material. Recall that we generated 154 test datasets each for MPE and MMAP (22 PCs $\times$ 7 $qr$ values). In the table, the number in the cell $(i,j)$ equals the number of times (out of 154) that the scheme in the $i$-th row was better in terms of average log-likelihood score than the scheme in the $j$-th column. The difference between 154 and the sum of the numbers in the cells $(i,j)$ and $(j,i)$ equals the number of times the scheme in the $i$-th row and $j$-th column had identical log-likelihood scores.

From the MPE contingency table given in Table \ref{tab:contingency-base}, we observe that \our is superior to \spn, \mle, and \seq approximations. The \seq approximation is slightly better than the \spn approximation, and \mle is the worst performing scheme. For the harder MMAP task, we see a similar ordering among the competing schemes (see \ref{tab:contingency-base}) with \our dominating other schemes. In particular, \our outperforms the \spn and \mle approximations in almost two-thirds of the cases and the \seq method in more than half of the cases.     

\input{content/tables/contingency-hill-climbing}

We also investigate the effectiveness of \our  and other baseline approaches when employed as initialization strategies for Hill Climbing Search. These findings are illustrated in the contingency tables given in Table \ref{tab:contingency-hill}. The results for \mpe are presented on the left side, while those for \mmap are presented on the right. Notably, \our 
%method showcases exceptional performance as an initialization technique for both \mpe and \mmap tasks. Specifically, it 
outperforms all other baseline approaches in nearly two-thirds of the experiments for both \mpe and \mmap tasks. These results demonstrate that \our can serve as an effective initialization technique for anytime local search-based algorithms.
%In this sequence of experiments, we initiate by providing contingency tables that encompass both our proposed \our method and the methodologies described in Section \ref{sec:exp-methods}. These outcomes are detailed in Table \ref{tab:contingency-base}. In this table, the value located at the $i^{th}$ row and $j^{th}$ column signifies the instances where the $i^{th}$ method exhibited superior performance to the $j^{th}$ method. Therefore, higher values within a row indicate that the corresponding method outperformed the competing methods. 

%The subset of experiments that remain is obtained by subtracting the combined values from the $i^{th}$ row and $j^{th}$ column, as well as the $j^{th}$ row and $i^{th}$ column, from the total count of experiments. This subset reflects instances in which the mean log likelihood scores exhibited equality between the two compared methods. 
\eat{We also present the results for the method where we incorporate entropy as a penalty, as introduced in Section \ref{sec:entropy}, referred to as \ourentropy and method that .} 

In Figure \ref{fig:performance_vs_spn}, via a heat-map representation, we show a more detailed performance comparison between \our and the \spn approximation, which is a widely used baseline for MPE and MMAP inference in PCs. In the heat-map representation, the y-axis represents the datasets (ordered by the number of variables), while the x-axis shows the query ratio. The values in each cell represent the percentage difference between the mean log-likelihood scores of \our and the \spn approximation. Formally, let $ll_{ssmp}$ and $ll_{max}$ denote the mean LL scores of \our and \spn approximation respectively, then the percentage difference is given by%formula is given in Equation \ref{eq:percent_diff}
\begin{equation}
\label{eq:percent_diff}
\begin{aligned}
\% \text{Diff.} = \frac{ll_{ssmp}-ll_{max}}{|ll_{max}|} \times 100
%\frac{(\text{\ourfig LL Mean} - \text{\spn LL Mean}) \times 100}{|\text{\spn LL Mean}|}
\end{aligned}
\end{equation}

\begin{figure}[thb!]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{content/figures/mpe_nn_spn_heatmap.pdf}
        \caption{\mpe}
        \label{fig:mpe_nn_vs_spn}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{content/figures/mmap_nn_spn_heatmap.pdf}
        \caption{\mmap}
        \label{fig:mmap_nn_vs_spn}
    \end{subfigure}
    
    \caption{Heat map showing the percentage difference in log-likelihood scores between \texttt{\our} and the \spn approximation. Blue color represents \spn's superiority (negative values), while red color represents \our's superiority (positive values).}
    \label{fig:performance_vs_spn}
\end{figure}

From the heatmap for MPE given in Figure \ref{fig:performance_vs_spn}(a), we observe that \our is competitive with the \spn approximation when the size of the query set is small. However, as the number of query variables increases, signaling a more challenging problem, \our consistently outperforms or has similar performance to the \spn method across all datasets, except for accidents, pumsb-star, and book.

The heatmaps for MMAP are illustrated in Figure \ref{fig:performance_vs_spn}(b). We see a similar trend as the one for MPE; \our remains competitive with the \spn approximation, particularly when the number of query variables is small. While \our outperforms (with some exceptions) the \spn approximation when the number of query variables is large.

Finally, we present inference times in the supplement. On average \our requires in the order of 7-10 micro-seconds for MMAP inference on an A40 GPU. The \spn approximation takes 7 milli-seconds (namely, \our is almost 1000 times faster). In comparison, as expected, the \seq and \mle approximations are quite slow, requiring roughly 400 to 600 milliseconds to answer MPE and MMAP queries. In the case of our proposed method (\our), during the inference process, the size of the SPN holds no relevance; its time complexity is linear in the size of the neural network. On the contrary, for the alternative methods, the inference time is intricately dependent on the size of the SPN.

\eat{
\sva{
\textbf{Can also include times for MPE - can select one of the following paragraphs. The first paragraph shows time for MMAP queries while the second paragraph shows time for both MPE and MMAP.}}

\sva{On average, the \our method proves to be the swiftest, requiring only 7.45 microseconds ($\mu$s) to solve an MMAP query. This showcases its remarkable efficiency compared to the \spn method, which has an average inference time of 6660.41 $\mu$s, making the \our method approximately 893.75 times faster. Additionally, the \our method demonstrates its rapidity by being around 58151.78 times faster than \mle, with an average inference time of 433358.17 $\mu$s, and a remarkable 85746.29 times faster than \seq, with an average query time of 638997.73 $\mu$s. }

\sva{On average, the \our method demonstrates remarkable speed, solving an MMAP query in just $7.45 \, \mu$s and an MPE query in $8.89 \, \mu$s. We present the speedup ratios and timings in the format "MMAP (MPE)" for subsequent methods. This efficiency shines in comparison to the \spn method, which requires an average inference time of $6.66041 \times 10^3$ ($1.274881 \times 10^4$) $\mu$s, making our \our method approximately $8.9375 \times 10^2$ ($1.43552 \times 10^3$) times faster. Moreover, our approach showcases its agility by surpassing the \mle method by approximately $5.815178 \times 10^4$ ($7.710485 \times 10^4$) times, with an average inference time of $4.3335817 \times 10^5$ ($6.84767 \times 10^5$) $\mu$s, and demonstrating a remarkable $8.574629 \times 10^4$ ($1.15797 \times 10^5$) times speedup over the \seq method, with an average query time of $6.3899773 \times 10^5$ ($1.028392 \times 10^6$) $\mu$s.}

Further elaboration on the running times can be found in the supplementary section.

Leveraging the full computational potential of GPU processing, the \our method enables queries to be resolved in real-time, contributing to its exceptional performance. Additional information regarding the inference times for all the methods will be elaborated upon in the supplementary section. This detailed analysis will offer a comprehensive understanding of the time taken by each method to perform inferences, providing a more thorough insight into their respective efficiencies and performance characteristics.
}

\subsection{Results on the CIFAR-10 dataset}
\input{content/tables/contingency-cifar-base}
%To assess \our's performance on additional real-world datasets, we embarked on experiments employing the 

We binarized the CIFAR-10 dataset \cite{krizhevskyLearningMultipleLayersFeaturesTinyImages} using a variational autoencoder having 512 bits. We then learned a PC for each of the 10 classes; namely, we learned a PC conditioned on the class variable. As mentioned earlier, we randomly set $70\%$ of the variables as query variables. The contingency table for CIFAR-10 is shown in Table \ref{tab:cifar10-base}. We observe that \our dominates all competing methods while the \seq approximation is the  second-best performing scheme (although note that \seq is computationally expensive).

%Our findings, as depicted in Table \ref{tab:cifar10-base}, consistently reveal the NN method's supremacy across all classes. This compellingly demonstrates the \our method's adeptness in surpassing alternative methodologies in real-world scenarios. Given its commendable performance and efficient execution time, \our method emerges as a robust candidate for diverse query computations on PCs.


%\subsection{Efficient Image Completion with Limited Data: MNIST and EMNIST Analysis}
%\label{subsec:exp_imagecompletion}
\subsection{Results on the MNIST and EMNIST datasets}
Finally, we evaluated \our on the image completion task using the Binarized MNIST \cite{salakhutdinov2008quantitative} and the EMNIST datasets \cite{cohenEMNISTExtensionMNISThandwrittenletters2017}. As mentioned earlier, we used the top 30\% of the image as evidence and estimated the bottom 70\% by solving the MPE task over PCs using various competing methods. 
% \input{content/tables/contingency_mnist-base}
% \vspace*{-5pt}
% \input{content/tables/contingency_emnist-base}
\input{content/tables/contingency-mnist-emnist-base}
The contingency tables for the MNIST and EMNIST datasets are shown in Table \ref{tab:mnist-base}. We observe that on the MNIST dataset, \our is better than all competing schemes on 9 out of the 10 PCs, while it is inferior to all on one of them. On the EMNIST dataset, \our is better than all competing schemes on 7 out of the 10 PCs, and inferior to all on one of the PCs. Detailed results on the image datasets, including qualitative comparisons, are provided in the supplement.

In summary, we find that, on average, our proposed method (\our) is better than other baseline MMAP approximations in terms of log-likelihood score. Moreover, it is substantially better than the baseline methods when the number of query variables is large. Also, once learned from data, it is also significantly faster than the other schemes.

%Once again, we employ contingency tables to gain insights into the performance of various methods. Let's begin by examining the contingency table for the MNIST and EMNIST datasets , as depicted in Table \ref{tab:mnist-base}. In the context of the ten classes within the MNIST dataset, the \our method outperformed all other baseline methods in nine instances. Shifting our focus to the EMNIST dataset, detailed results are presented on the right side of the table. Within this dataset, featuring eight selected classes, the \our method exhibited superior performance compared to all other baselines in seven cases. This demonstration underscores the applicability of the \our method in real-world scenarios, such as image completions, where it excels by offering enhanced performance and expedited results compared to other inference techniques employed in probabilistic contexts. In consideration of space limitations, we present qualitative results for the MNIST and EMNIST datasets in the supplementary section.

%\subsection{Summary}

\eat{For both datasets, the \ourtt method outperforms the \our method in 9 out of 10 cases and 3 out of 8 cases, respectively. Similarly, the \ourentropy method outperforms the \our method three times for both datasets, showcasing consistent trends across the experiments.}

\eat{
% Qualitative Results for MNIST and EMNIST
\begin{figure}[h]
    \centering
    \setlength{\tabcolsep}{10pt} % Adjust spacing between subfigures
    
    \begin{tabular}{@{}cc@{}}
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/mnist_5_623.png}
            \caption{MNIST Digit 5}
        \end{subfigure} &
        
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/mnist_6_589.png}
            \caption{MNIST Digit 6}
        \end{subfigure} \\
        
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/mnist_8_38.png}
            \caption{MNIST Digit 8}
        \end{subfigure} &
        
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/mnist_9_422.png}
            \caption{MNIST Digit 9}
        \end{subfigure} \\
    \end{tabular}
    
    \vspace{1em} % Add vertical spacing for visual balance
    
    \begin{tabular}{@{}cc@{}}
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/emnist_1_420.png}
            \caption{EMNIST Character A}
        \end{subfigure} &
        
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/emnist_3_526.png}
            \caption{EMNIST Character C}
        \end{subfigure} \\
        
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/emnist_19_388.png}
            \caption{EMNIST Character S}
        \end{subfigure} &
        
        \begin{subfigure}{0.42\columnwidth}
            \includegraphics[width=\linewidth]{content/images/emnist_22_763.png}
            \caption{EMNIST Character V}
        \end{subfigure} \\
    \end{tabular}
    
    \caption{Image Completions for MNIST and EMNIST datasets. First image: Original. Second image: \spn Completion. Third image: \our Completion. The gray line separates evidence (above) from query (below).}
    \label{fig:image-completion}
\end{figure}

Qualitative image completions for MNIST and EMNIST datasets are presented in Figure \ref{fig:image-completion}. Beginning with the original image as the initial reference, followed by the \spn method's completion attempt, and culminating in our novel \our method's completion. Specifically, characters such as 8, 9, A, and S exhibit discontinuities in their \spn-generated completions, as the lower portions fail to align with their upper counterparts seamlessly. This showcases the arduous nature of the challenge and underscores the limitations of the \spn method in handling such intricate tasks. In stark contrast, the proposed \our method offers a remarkable improvement in completion quality. It adeptly addresses the difficulties posed by limited available information and generates reconstructions that are not only smoother but also exhibit a remarkable coherence. This highlights \our method's efficacy in real-world scenarios with limited information but extensive query needs.}

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{content/figures/nist/mnist.pdf}
%         \caption{MNIST -ve Log Likelihood Scores}
%         \label{fig:mpe_nn_vs_spn}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{content/figures/nist/emnist.pdf}
%         \caption{EMNIST -ve Log Likelihood Scores}
%         \label{fig:mmap_nn_vs_spn}
%     \end{subfigure}
    
%     \caption{Performance Comparison}
%     \label{fig:performance_vs_spn}
% \end{figure}

\eat{
\subsection{Training}
To ensure that the NN performs at least as good as the PC on approximating MMAP, we perform a pretraining step.
\subsection{Results}

A fast approximate method to solve \ref{eqn:mmap} is to replace the inner summation by a maximization over $\mathbf{h}$. This is equivalent to switching sum nodes to max nodes in a PC and then performing a bottom pass followed by a top-down pass to construct an assignment $\langle \mathbf{q}^*,\mathbf{h}^*\rangle$. The MMAP solution is then approximated by the partial assignment $\mathbf{q}^*$, ignoring $\mathbf{h}^*$.
\subsubsection{To Discuss}
\begin{itemize}
    \item Overfitting? MMAP value of NN $>$ MMAP value of SPN on training data, but the opposite relation holds in most of the test samples. 
    \item What kind of regularizations can we use? 
\end{itemize}
}

==> content/intro_new.tex <==
\section{Introduction}\label{sec:intro}
Probabilistic circuits (PCs) \cite{choi2020probabilistic} such as sum-product networks (SPNs) \cite{poon2011sum}, arithmetic circuits \cite{darwiche2003differential}, \verify{bounded depth AND/OR graphs \cite{dechter2007and}}, cutset networks \cite{rahman2014cutset}, and probabilistic sentential decision diagrams \cite{kisa2014probabilistic}  represent a class of \textit{tractable probabilistic models} which compactly encode the joint probability distribution over random variables in a domain. The three most common inference tasks performed over PCs are: 1) computing marginal probabilities (MAR) over a subset of random variables with or without evidence, known as the \textit{sum-inference} task, 2) given observation or evidence over a subset of variables, finding the most-probable-explanation (MPE/MAP) or assignment to the rest of the variables, also known as the \textit{max-inference} task, and finally, 3) given observation (evidence) over a subset of variables, finding the marginal maximum-a-posteriori (MMAP) assignment to some other subset of variables by marginalizing out the rest of the unobserved variables. This task is also known as the max-and-sum or \textit{mixed-inference} task. Unlike arbitrary structured Bayesian networks and Markov networks in which all of these inference tasks are NP-hard to solve, all PCs including PCs with latent variables allow linear time computation of the MAR task and PCs without any latent variables, e.g., cutset networks, AND/OR graphs, etc. admit tractable MPE/MAP inference. 
\eat{Even though all of these models admit linear time computation of marginal probabilities (MAR task), only some of them, specifically those without any latent variables, e.g., cutset networks, AND/OR graphs, arithmetic circuits, etc. admit tractable most probable explanation (MPE) inference.}However, none of these expressive PCs can efficiently solve the MMAP task, a task that combines MAR and MPE inference \cite{peharz2015foundations}. In fact, it remains an NP-hard problem in these models, just like in BNs and MNs. 

\eat{More specifically, the difference between MPE and MMAP is that given observations over a subset of variables, MPE finds the most-likely assignment to all other variables while MMAP finds such assignment only over a subset of these variables while marginalizing over the rest.} 

Existing methods that try to exactly solve MMAP queries over PCs are based on branch-and-bound search \cite{maua2020two, mei2018maximum} or circuit transformations (pruning) \cite{choi2022solving}. These methods are often impractical for answering these queries in real-time, and therefore approximate schemes are readily adopted. Approximate solutions can be obtained in several ways, e.g., converting the given MMAP task to an MPE task defined over both the query and unobserved variables, as done in SPNs and other mixture models \cite{poon2011sum}, or compiling the original model with unobserved variables to a model with observed variables only that is tractable for MPE \cite{rahman2019look}. Although these approaches can provide fast answers at query time, they are often far from the true optimal and can require an extra model transformation step. In this paper, we address the problem of improving the accuracy and efficiency of the MMAP task in PCs by using deep neural networks.

Deep neural networks have been used in the past to improve the representational power of PCs. For example, conditional PCs like conditional cutset networks \cite{rahman2019cutset, dong2022conditionally} and conditional sum-product-networks \cite{shao2020conditional} incorporate NNs in their structure to fit arbitrary complex conditional distributions. Their primary purpose is to act as discriminative classifiers and accurately predict conditional probabilities over random variables given evidence. This has led to significant boost in the performance of PCs in representing tractable, expressive conditional distributions.  

Recently, several works have shown promising results in using NNs to solve both constrained and unconstrained optimization problems \cite{park2022self} and the references therein. The high level idea is given data, train NNs, either in a supervised manner or in a self-supervsed manner, to predict high-quality, near-optimal solutions to future  problems in the domain of interest. A number of reasons have motivated this idea of \textit{learning to optimize} using NNs: 1) NNs are good at approximating complex functions (distributions), 2) once trained, they can be faster at answering such queries than search based approaches, and 3) with ample data, NNs can learn accurate mappings of inputs to corresponding outputs. This has led researchers to employ NNs to compute answers to probabilistic queries like MARs and MPEs on BNs and MNs \cite{yoon2019inference, cui2022variational}\eat{that can be cast as optimization problems, for example, using variational inference techniques to compute MARs and MPEs in PGMs \cite{??}}. To the best of our knowledge, there is no prior work on solving MMAP in BNs, MNs or PCs using deep neural networks.  

We make the following contributions in this paper: 1) we propose to learn a neural network approximator for solving the MMAP task in PCs, 2) leveraging the tractability of these expressive models, we devise a loss function that can efficiently be evaluated at each iteration of gradient descent, 3) our method trains an NN in a self-supervised manner without having to rely on pre-computed solutions to arbitrary MMAP problems, 4) empirical results on several state-of-the-art PCs show that neural approximators can significantly improve the accuracy of MMAP in PCs. 

    \eat{Note that, although the MPE task ($|Z| = 0$) is tractable in PCs without latent variables, for example cutset networks, it is an NP-hard problem in PCs with latent variables e.g. sum-product networks and many popular mixture models, that is, MPE becomes an MMAP task in PCs with latent variables and unfortunately inherits its computational complexities.
    \eat{The three most common inference tasks performed over PCs are: 1) computing the marginal probability (MAR) over a subset of random variables with or without evidence, 2) given evidence over a subset of variables, finding  the most-probable-explanation (MPE) or assignment to the rest of the variables, and 3) given evidence over a subset of variables, finding the maximum-a-posteriori (MMAP) assignment to some other subset of variables from the distribution that is consistent with the given evidence and obtained through marginalizing out the rest of the unobserved variables.} 

    
    }
   



==> content/method-removed-text.tex <==

\eat{probabilistic circuit where we replace every leaf node $Q_i$ such that $Q_i \in \mathbf{Q}$ by $q_i^c$ and $\neg Q_i$ by $1-q_i^c$. More formally,
\paragraph{Definition 1.}
Let $\mathcal{M}$ be a PC over variables $\mathbf{X}=\mathbf{E} \cup \mathbf{Q} \cup \mathbf{H}$ where $\mathbf{E},\mathbf{Q},\mathbf{H}$ is a partition of $\mathbf{X}$. A $\mathbf{Q}$-PC of $\mathcal{M}$, denoteed by $\mathcal{M}^{\mathbf{q}}$ is a PC that is obtained by replacing each variable $Q_i \in \mathbf{Q}$ by a continuous variable $Q_i^c$ having domain $[0,1]$ and all indicator functions $[Q_i=1]$ and $[Q_i=0]$ where $Q_i \in \mathbf{Q}$ by corresponding continuous functions that equal $q_i^c$ and $1-q_i^c$ respectively where $q_i^c \in [0,1]$. 
%\end{definition}
\newcommand{\todo}[1]{\textit{Todo}}

By construction, if a PC $\mathcal{M}$ is smooth and decomposable then the $\mathbf{Q}$-PC $\mathcal{M}^{\mathbf{q}}$ of $\mathcal{M}$ is also smooth and decomposable. Given an assignment $\mathbf{e}_i$ and $\mathbf{q}_i^c$, let $\mathcal{M}^{\mathbf{q}}(\mathbf{e}_i,\mathbf{q}_i^c)$ denote the value of root node of $\mathcal{M}^{\mathbf{q}}$ obtained by setting all hidden variables to $1$, all indicator functions corresponding to variables in $\mathbf{E}$ w.r.t. the assignment $\mathbf{e}_i$, and evaluating the continuous functions using values from $\mathbf{q}_i^c$. Figure \ref{fig:1}(b) shows a $\mathbf{Q}$-PC of the PC give in Figure \ref{fig:1}(c). The reader can verify that given evidence \todo{} and assignment $\todo{}$ to the query variables, the value of the root node of the  $\mathbf{Q}$-PC given in \ref{fig:1}(b) is \todo{}.

Intuitively, $\mathcal{M}^{\mathbf{q}}(\mathbf{e}_i,\mathbf{q}_i^c)$ is a continuous approximation of 
$\mathcal{M}(\mathbf{e}_i,\mathbf{q}_i)$, and the difference between the two is minimized iff  $\mathbf{q}_i^c=\mathbf{q}_i$. Moreover, since the set of continuous assignments includes the discrete assignments, it follows that:
\[ \max_\mathbf{q} \mathcal{M}(\mathbf{q}|\mathbf{e}) \leq \max_{\mathbf{q}^c} \mathcal{M}^\mathbf{Q}(\mathbf{q}^c|\mathbf{e})\]

Based on the discussion above, we propose the following loss function:
\begin{align}
\label{eq:loss_function}
    \mathcal{L}(\mathbf{q}^c|\mathbf{e}) = -\ln \mathcal{M}^\mathbf{Q}(\mathbf{q}|\mathbf{e})
\end{align}

We can show that the loss function is smooth and differentiable, and if the PC is smooth and decomposable, then the partial derivative w.r.t. $q_i$ can be computed in linear time in the size of the PC. Figure \ref{fig:1}(c) shows the computation of partial derivative of the loss function w.r.t. $Q_2$. More formally,
\begin{prop}
Given a smooth and decomposable PC $\mathcal{M}$, the partial derivative of $\mathcal{L}(\mathcal{q}^c|\mathbf{e})$ given in equation \eqref{eq:loss_function} w.r.t. $Q_i$ is given by
\begin{align}
\label{eq:derivative}
    \frac{\partial \mathcal{L}(\mathbf{q}^c|\mathbf{e})}{\partial q_i} = -\frac{\mathcal{M}^\mathbf{Q}(\mathbf{q}_i,q_i=1|\mathbf{e})}{\mathcal{M}^\mathbf{Q}(\mathbf{q}|\mathbf{e})}
\end{align}
\end{prop}
Since the partial derivative requires only two evaluations of the PC, it can be computed in linear time in the size of the network. Thus, our loss function ensures that each iteration of stochastic gradient descent takes linear time in the size of the neural network and the PC. 



Then, we propose to use the following loss function:
\begin{align}\label{eqn:loss}
    \mathcal{L}(\hat{\mathbf{q}}_i|\mathbf{e}_i) & = -\ln P(\hat{\mathbf{q}}_i|\mathbf{e}_i)\nonumber\\
    & = -\ln \sum_{\mathbf{h}} P(\hat{\mathbf{q}}_i,\mathbf{h}|\mathbf{e}_i)
\end{align}

We assume that each $\mathbf{e}_i \in \mathcal{D}$ has been sampled from the distribution $P(\mathbf{E}) = P(E_1)\prod_{i=2}^{N}P(E_i|E_{1:i-1})$. Each conditional distribution $P(E_i|E_{1:i-1})$ can be computed exactly by performing tractable marginal inference over the given PC. At any given iteration, the NN predicts an MMAP assignment $\hat{\mathbf{q}}_i = f_\theta(\mathbf{e}_i)$. We define a loss $\ell_i(\mathbf{e}_i, \hat{\mathbf{q}}_i)$ for each predicted assignment as the unnormalized negative (log) probability $-P(\mathbf{e}_i, \hat{\mathbf{q}}_i)$ according to the given PC. The total loss $\mathcal{L}(.)$ to be minimized can therefore be defined as the average of these individual losses. Mathematically, 
\begin{align}\label{eqn:loss}
    \mathcal{L}(\mathcal{D}) & = \frac{1}{n}\sum_{i=1}^n\ell_i(\mathbf{e}_i, \hat{\mathbf{q}}_i) =  \frac{1}{n}\sum_i^n-P(\mathbf{e}_i, \hat{\mathbf{q}}_i)\nonumber\\
    & = -\frac{1}{n}\sum_{i=1}^n\bigg(\sum_\mathbf{h}P(\mathbf{e}_i,\hat{\mathbf{q}}_i,\mathbf{h})\bigg) 
\end{align}
As mentioned earlier, since the neural network outputs a continuous quantity

Since each predicted assignment $\hat{\mathbf{q}}_i = \{\hat{q}_{1,i},\ldots,\hat{q}_{M,i}\}$ is a continuous vector in $[0,1]^M$, loss $\ell(\mathbf{e}_i, \hat{\mathbf{q}}_i)$ is a linear approximation to the ILP formulation of the MMAP problem given by $\mathbf{e}_i$. Finally, computing the gradients $\frac{\partial\mathcal{L}}{\partial\hat{\mathbf{q}}_i}$'s can be done efficiently since loss $\mathcal{L}(.)$ is tractable; each $\ell_i(.)$ is bounded by the size of the PC. 
}


\eat{
Formally, we can achieve this by solving the following constrained minimization task:
\begin{align}
 \nonumber
    \text{minimize} -\ln v'(r,(\mathbf{e},\mathbf{q}^c)\text{ s.t.}\; \\
    - \mathbf{q}^c_j \log(\mathbf{q}^c_j) -  (1-\mathbf{q}^c_j) \log(1-\mathbf{q}^c_j) \leq \epsilon; \;\text{for}\; j=1,\ldots,M
\end{align}
We can convert the constrained minimization problem to an unconstrained one by adding a hyperparameter $\alpha_j$ that penalizes each constraint violation in a soft manner. More formally, using a penalty $\alpha_j\geq 0$ for each constraint, we get
\begin{align}
 \nonumber
    \text{minimize} -\ln v'(r,(\mathbf{e},\mathbf{q}^c) - \left (\sum_{j=1}^{M} \alpha_i 
     \mathbf{q}^c_j \log(\mathbf{q}^c_j) +  (1-\mathbf{q}^c_j) \log(1-\mathbf{q}^c_j) \right )
\end{align}


\subsubsection{On Finding Discrete Solutions}
\label{sec:entropy}
One approach to obtain discrete MMAP solutions is to round each continuous output $\hat{q}_i\in[0,1]$ to the nearest integer. This approach may result in inaccurate sub-optimal solutions. We propose to add the following penalty to the loss $\mathcal{L}(.)$ that encourages discrete solutions by minimizing the sum of the entropies over the output variables.
\begin{equation*}
    \mathcal{L}(\mathcal{D}) - \alpha \sum_{j=1}^n\sum_{i=1}^M\bigg(\hat{q}_{i,j}\log(\hat{q}_{i,j}) + (1-\hat{q}_{i,j})\log(1-\hat{q}_{i,j})\bigg)
\end{equation*}
where $\alpha$ is a hyperparameter and each $\hat{q}_{i,j}$ is the predicted quantity $\hat{P}(Q_i = 1|\mathbf{e}_j)$ ($i^{th}$ output) on the $j^{th}$ input. 

\sva{Need to add a subsubsection for case where we also train on the test set}

}

==> content/method-vibhav.tex <==
\section{A Neural Optimizer for MMAP in PC\text{s}}\label{sec:method}
In this section, we introduce a learning-based approach that uses a neural network (NN) to approximately solve the MMAP problem in PCs. Formally, the NN represents a function $f_\theta(.)$ that is parameterized by $\theta$, and takes an assignment $\mathbf{e}$ over the evidence variables as input and outputs an assignment $\mathbf{q}$ over the query variables. Our goal is to design \emph{generalizable, continuous loss functions} for updating the parameters of the NN such that once learned, at test time, given an assignment $\mathbf{e}$ to the evidence variables as input, the NN outputs near-optimal solutions to the MMAP problem.

For simplicity, we assume that the sets of evidence $\left (\mathbf{E} = \{E_i\}_{i=1}^N \right )$ and query $\left (\mathbf{Q}=\{Q_j\}_{j=1}^M \right )$ variables are known \textit{a priori} and do not change at both training and test time. In the supplement, we propose a generalization of our approach that can efficiently handle variable length, arbitrarily chosen evidence, and query sets. Also, note that our proposed method does not depend on the particular NN architecture used and we only require that each output node is a continuous quantity in the range $[0,1]$ and uses a differentiable activation function (e.g., the sigmoid function). 

%Next, we describe how to train the parameters of $f_\theta(.)$ from data. 

%Next, we describe our proposed approach for training the parameters of $f_\theta(.)$ from data.

%that is an optimal solution (in practice a close to optimal solution) to the MMAP problem defined in \ref{eqn:mmap}.

%to predict answers to marginal MAP queries in PCs.  Formally, a \textit{neural network optimizer} for the MMAP task over a given PC is a deep neural network $f_\theta(.)$ parameterized by $\theta$ which takes as input an (possibly encoded) assignment $\mathbf{e}$ over the evidence variables and outputs an assignment $\hat{\mathbf{q}}$ over the query variables that is an optimal solution (in practice a close to optimal solution) to the MMAP problem defined in \ref{eqn:mmap}. 

%For now, we will assume that the sets of evidence ($\mathbf{E} = \{E_i\}_1^N$), query ($\mathbf{Q}=\{Q_j\}_1^M$) and hidden ($\mathbf{H}=\{H_k\}_1^K$) variables are all fixed and known \textit{a priori} for each MMAP task posed to the PC. In the supplement, we propose a generalization to efficiently handle variable length, arbitrarily chosen evidence, query and hidden variables. 



We can learn the parameters of the given NN either in a \textit{supervised} manner or in a \textit{self-supervised} manner. However, the supervised approach is impractical as described below. 

In the supervised setting, we assume that we are given training data $\mathcal{D} = \{\langle \mathbf{e}_1, \mathbf{q}_1^*\rangle,\ldots,\langle \mathbf{e}_n, \mathbf{q}_n^*\rangle\}$, where each input $\mathbf{e}_i$ is an assignment to the evidence variables, and each output (label) $\mathbf{q}_i^*$ is an optimal solution to the corresponding MMAP task, namely $\mathbf{q}_i^*=\texttt{MMAP}(\mathbf{Q},\mathbf{e}_i)$. We then use supervised loss functions such as the mean-squared-error (MSE) $\sum_i(\mathbf{q}^*_i - \mathbf{q}_i^c)^2/n$ and the mean-absolute-error (MAE) $\sum_i|\mathbf{q}^*_i - \mathbf{q}_i^c|/n$ where $\mathbf{q}_i^c$ is the predicted assignment (note that $\mathbf{q}_i^c$ is continuous), and standard gradient-based methods to learn the parameters. Although supervised approaches allow us to use simple-to-implement loss functions, they are \textit{impractical} for large PCs because they require access to the exact solutions to several intractable MMAP problems\footnote{Note that the training data used to train the NN in the supervised setting is different from the training data used to learn the PC. In particular, in the data used to train the PC, the assignments to the query variables $\mathbf{Q}$ may not be optimal solutions of $\texttt{MMAP}(\mathbf{Q},\mathbf{e})$.}. We therefore propose to use a \textit{self-supervised approach}. 

%we cannot use the assignments  $\mathbf{q}^*_i$ given in the training data to learn the parameters of $f_\theta(.)$ in a supervised manner because  $\mathbf{q}$ is not an optimal solution to the sampled $\mathbf{e}$.}. \marginpar{TR:See footnote text} We therefore propose a self-supervised approach in the next section. 

%At each iteration, during training by gradient descent, the NN predicts an MMAP assignment $\hat{\mathbf{q}}_i = f_\theta(\mathbf{e}_i)$ for each input $\mathbf{e}_i\in\mathcal{D}$ according to its current set of parameters. It then back-propagates a supervised loss (error) like the mean-squared-error (MSE) $\frac{\sum_i(\mathbf{q}^*_i - \hat{\mathbf{q}}_i)^2}{n}$ or the mean-absolute-error (MAE) $\frac{\sum_i|\mathbf{q}^*_i - \hat{\mathbf{q}}_i|}{n}$ to update its parameters. This iterative minimization of the loss continues until convergence. Note that during such supervised training the PC under consideration is never queried. Although such supervised approaches allow us to use simple to implement loss functions, they require access to the exact solutions to several MMAP problems, potentially over high-dimensions, which are infeasible to obtain in practice\footnote{Note that we cannot use the assignment to $\mathbf{q}$ given in the training data to learn the parameters of $f_\theta(.)$ in a supervised manner because  $\mathbf{q}$ is not an optimal solution to the sampled $\mathbf{e}$.}. \marginpar{TR:See footnote text} We therefore propose a self-supervised approach in the next section. 

% cite - didn't know two citations here
\subsection{A Self-Supervised Loss Function for PCs}
In the self-supervised setting, we need access to training data in the form of assignments to the evidence variables, i.e., $\mathcal{D}' = \{\mathbf{e}_1,\ldots,\mathbf{e}_n\}$. Since smooth and decomposable PCs admit perfect sampling, these assignments can be easily sampled from the PC via top-down AND/OR sampling \cite{gogate&dechter12}. The latter yields an assignment $\mathbf{x}$ over all the random variables in the PC. Then we simply project $\mathbf{x}$ on the evidence variables $\mathbf{E}$ to yield a training example $\mathbf{e}$. Because each training example can be generated in time that scales linearly with the size of the PC, our proposed self-supervised approach is significantly more scalable than the supervised approach.

Let $\mathbf{q}^c$ denote the MMAP assignment predicted by the NN given evidence $\mathbf{e} \in \mathcal{D}'$ where $\mathbf{q}^c \in [0,1]^{M}$. In MMAP inference, given $\mathbf{e}$, we want to find an assignment $\mathbf{q}$ such that $\ln \texttt{p}_{\mathcal{M}}(\mathbf{e},\mathbf{q})$ is maximized, namely, $-\ln \texttt{p}_{\mathcal{M}}(\mathbf{e},\mathbf{q})$ is minimized. Thus, a natural loss function that we can use is  $-\ln \texttt{p}_{\mathcal{M}}(\mathbf{e},\mathbf{q})$. Unfortunately, the NN outputs a continuous vector $\mathbf{q}^c$ and as a result $\texttt{p}_{\mathcal{M}}(\mathbf{e},\mathbf{q}^c)$ is not defined. Therefore, we cannot use $-\ln \texttt{p}_{\mathcal{M}}(\mathbf{e},\mathbf{q}^c)$ as a loss function.



One approach to circumvent this issue is to use a threshold (say $0.5$) to convert each continuous quantity in the range [0,1] to a binary one. A problem with this approach is that the threshold function is not differentiable. 

Therefore, we propose to construct a smooth, differentiable loss function that given $\mathbf{q}^c=(q_1^c,\ldots,q_M^c)$ approximates $-\ln \texttt{p}_{\mathcal{M}}(\mathbf{e},\mathbf{q})$ where $\mathbf{q}=(q_1=[q_1^c>0.5],\ldots,q_M=[q_M^c>0.5])$ and $[q_i^c>0.5]$ is an indicator function which is $1$ if $q_i^c>0.5$ and $0$ otherwise. The key idea in our approach is to construct a new PC, which we call \textit{Query-specific PC} (QPC) by replacing all binary leaf nodes associated with the query variables in the original PC, namely those labeled by $Q$ and $\neg Q$ where $Q \in \mathbf{Q}$, with continuous nodes $Q^c \in \mathbb{R}$ and $\neg Q^c \in \mathbb{R}$. Then our proposed loss function is obtained using value computations at the \textit{root node} of the QPC via a simple modification of the \textit{leaf function} of the PC. At a high level, our new leaf function assigns each leaf node labeled by $Q_j^c$ such that $Q_j \in \mathbf{Q}$ to its corresponding estimate $q_j^c$, obtained from the NN and each leaf node labeled by $\neg Q_j^c$ such that $Q_j \in \mathbf{Q}$ to $1-q_j^c$. 
%Here, the notation $\mathbf{q}_j^c$ denotes the $j$-th element of the vector $\mathbf{q}^c$ and corresponds to a continuous estimate of the value of the binary variable $Q_j$. 

%Our proposed loss function is obtained at the \textit{root node} of the PC via a simple modification of its \textit{leaf function}. At a high level, our new leaf function assigns each leaf node labeled by $Q_j$ such that $Q_j \in \mathbf{Q}$ to its corresponding estimate $\mathbf{q}_j^c$ from the neural network and each leaf node labeled by $\neg Q_j$ such that $Q_j \in \mathbf{Q}$ to $1-\mathbf{q}_j^c$. Here, the notation $\mathbf{q}_j^c$ denotes the $j$-th element of the vector $\mathbf{q}^c$ and corresponds to a continuous estimate of the value of the binary variable $Q_j$. 

%Therefore, we propose to construct a smooth, differentiable function that is obtained at the \textit{root node} of the PC via a simple modification of the \textit{leaf function}. At a high level, our new leaf function assigns each leaf node labeled by $Q_j$ such that $Q_j \in \mathbf{Q}$ to its corresponding estimate $\mathbf{q}_j^c$ from the neural network and each leaf node labeled by $\neg Q_j$ such that $Q_j \in \mathbf{Q}$ to $1-\mathbf{q}_j^c$. Here, the notation $\mathbf{q}_j^c$ denotes the $j$-th element of the vector $\mathbf{q}^c$ and corresponds to a continuous estimate of the value of the binary variable $Q_j$. 

Formally, for the QPC, we propose to use leaf function $l'(n,(\mathbf{e},\mathbf{q}^c))$ defined as follows:
\begin{enumerate}
    \item If the label of $n$ is $Q_j^c$ such that $Q_j \in \mathbf{Q}$ then $l'(n,(\mathbf{e},\mathbf{q}^c))=q^c_{j}$.
    \item If $n$ is labeled by $\neg Q_j^c$ such that $Q_j \in \mathbf{Q}$ then $l'(n,(\mathbf{e},\mathbf{q}^c))=1-q^c_{j}$.
    \item If $n$ is labeled by $E_k$ such that $E_k \in \mathbf{E}$ and the assignment $E_k=0$ is in $\mathbf{e}$ then $l'(n,(\mathbf{e},\mathbf{q}^c))=0$.
    \item If $n$ is labeled by $\neg E_k$ such that $E_k \in \mathbf{E}$ and the assignment $E_k=1$ is in $\mathbf{e}$ then $l'(n,(\mathbf{e},\mathbf{q}^c))=0$.
    \item If conditions (1)-(4) are not met then $l'(n,(\mathbf{e},\mathbf{q}^c))=1$.
\end{enumerate}
The value of each node $n$ in the QPC, denoted by $v'(n,(\mathbf{e},\mathbf{q}^c))$ is given by a similar recursion to the one given in Eq. \eqref{eq:recursion} for PCs, except that the leaf function $l(n,\mathbf{q})$ is replaced by the new (continuous) leaf function $l'(n,(\mathbf{e},\mathbf{q}^c))$. Formally, $v'(n,(\mathbf{e},\mathbf{q}^c))$ is given by
%\begin{equation}
%\small
    \begin{multline}
    \label{eq:recursion2}
    v'((n,(\mathbf{e},\mathbf{q}^c))
    \\
    =\left \{ \begin{array}{ll}
    l' (n,(\mathbf{e},\mathbf{q}^c))& \text{if $n \in \mathcal{L}$}\\
    \sum_{m \in \texttt{ch}(n)} \omega(m,n) v'(m,(\mathbf{e},\mathbf{q}^c)) & \text{if $n \in \mathcal{S}$}\\
    \prod_{m \in \texttt{ch}(n)} v'(n,(\mathbf{e},\mathbf{q}^c)) &\text{if $n \in \mathcal{P}$}
    \end{array} \right .
    \end{multline}
    %\end{split}
%\normalsize
%\end{equation}
Let $r$ denote the root node of $\mathcal{M}$, then we propose to use $-\ln v'(r,(\mathbf{e},\mathbf{q}^c))$ as a loss function. 
\begin{example}
    Figure \ref{fig:example}(b) shows the QPC corresponding to the PC shown in Figure \ref{fig:example}(a). We also show value computations for the assignment $(X_3^c=0.99,X_4^c=0.05)$.% over the QPC. 
\end{example}

\subsection{Tractable Gradient Computation}
%\subsubsection{Gradient Computation}
Our proposed loss function is smooth and continuous because by construction, it is a negative logarithm of a \textit{multilinear function} over $\mathbf{q}^c$. Next, we show that the partial derivative of the function w.r.t. $q_j^c$ can be computed in linear time in the size of the QPC\footnote{Recall that $q_j^c$ is an output node of the NN and therefore backpropagation over the NN can be performed in time that scales linearly with the size of the NN and the QPC}. More specifically, in order to compute the partial derivative of QPC with respect to $\mathbf{q}_j^c$, we simply have to use a new leaf function which is identical to $l'$ except that if the label of a leaf node $n$ is $Q_j^c$ then we set its value to $1$ (instead of $q_j^c$) and if it is $\neg Q_j^c$ then we set its value $-1$ (instead of $1-q_j^c$). We then perform bottom-up recursive value computations over the QPC and the value of the root node is the partial derivative of the QPC with respect to $\mathbf{q}_j^c$. In summary, we can show that (proof is provided in the appendix):
\begin{proposition}
    The gradient of the loss function $-\ln v'(r,(\mathbf{e},\mathbf{q}^c))$ w.r.t. $\mathbf{q}_j^c$ can be computed in time and space that scales linearly with the size of $\mathcal{M}$.
\end{proposition}

\begin{example}
The partial derivative of the QPC given in figure \ref{fig:example}(b) w.r.t. $x_3^c$ given $(X_3^c=0.99,X_4^c=0.05)$ can be obtained by setting the leaf nodes $X_3^c$ to $1$ and $\neg X_3^c$ to $-1$, assigning all other leaves to the values shown in Figure \ref{fig:example}(b) and then performing value computations. After the value computation phase, the value of the root node will equal the partial derivative of the QPC w.r.t. $x_3^c$.
 %   Figure \ref{fig:example}(c) shows the 
\end{example}
%The partial derivative of the QPC given in figure \ref{fig:example}(b) w.r.t. $x_3^c$ can be obtained by setting leaf nodes $X_3^c$ to $1$ and $\neg X_3^c$ to $-1$, keeping all other leaves to their previous value and performing value computations. 


\subsection{Improving the Loss Function}
%A key feature of our proposed loss function is that its optimal value is guaranteed to be smaller than or equal to the negative logarithm of the MMAP value (the latter yields an optimal MMAP assignment). This lower bounding property follows from the fact that the set of continuous assignments includes the discrete assignments. Formally,
%
As mentioned earlier, our proposed loss function is a continuous approximation of the discrete function $-\ln v(r,(\mathbf{e},\mathbf{q}))$ where $\mathbf{q}=(q_1=[q_1^c>0.5],\ldots,q_M=[q_M^c>0.5])$ and the difference between the two is minimized iff $\mathbf{q}=\mathbf{q}^c$. Moreover, since the set of continuous assignments includes the discrete assignments, it follows that:
\begin{align} 
\label{eq:loss-function} 
\min_{\mathbf{q}^c} \left \{ -\ln v'(r,(\mathbf{e},\mathbf{q}^c)) \right \} \leq \min_{\mathbf{q}} \left \{-\ln v(r,(\mathbf{e},\mathbf{q})) \right \}   
\end{align}
Since the right-hand side of the inequality given in \eqref{eq:loss-function} solves the MMAP task, we can improve our loss function by tightening the lower bound. This can be accomplished using an entropy-based penalty, controlled by a hyper-parameter $\alpha>0$, yielding the loss function
\begin{align}
\nonumber
    \ell(\mathbf{q}^c) =
    -\ln v'(r,(\mathbf{e},\mathbf{q}^c))-\\ 
    \label{eqn:loss} \alpha \sum_{j=1}^{M} 
     q^c_j \log(q^c_j) +  (1-q^c_j) \log(1-q^c_j) 
\end{align}  
%We propose to tighten the lower bound by moving each continuous quantity output by the neural network towards $0$ or $1$ (namely towards discrete values). 

%conclude that after optimization via a gradient-based algorithm, our proposed method approximates the 
%will yield a continuous lower bound on the true loss.

%An issue with our proposed continuous loss function is that although its optima lower bounds the optima of the true (discrete) loss, the gap between the two can be quite large. Moreover, since discrete outputs are desired, it is unclear what threshold should one use in order to convert the continuous assignment to a discrete one. We therefore propose to use a set of entropy-based constraints which encourages discrete solutions and penalizing them using a hyperparameter $\alpha>0$. Formally, we propose to use the following loss function:
%\[-\ln v'(r,(\mathbf{e},\mathbf{q}^c) - \alpha \sum_{j=1}^{M} 
 %    \mathbf{q}^c_j \log(\mathbf{q}^c_j) +  (1-\mathbf{q}^c_j) \log(1-\mathbf{q}^c_j)   \]
The second term in the expression given above is minimized when each $q^c_j$ is closer to $0$ or $1$ and is maximized when $q^c_j=0.5$. Therefore, it encourages 0/1 (discrete) solutions. The hyperparameter $\alpha$ controls the magnitude of the penalty. When $\alpha=0$, the above expression finds an assignment based on the continuous approximation $-\ln v'(r,(\mathbf{e},\mathbf{q}^c))$. On the other hand, when $\alpha=\infty$ then only discrete solutions are possible yielding a non-smooth loss function. $\alpha$ thus helps us trade the smoothness of our proposed loss function with its distance to the true loss.


==> content/prelim-vibhav.tex <==
\section{Preliminaries}
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
    \resizebox{0.95\textwidth}{!}{\input{figures/pc1}}
    \caption{PC}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
    \resizebox{0.95\textwidth}{!}{\input{figures/pc2}}
    \caption{QPC}
    \end{subfigure}
    \caption{(a) An example smooth and decomposable PC. The figure also shows value computation for answering the query $\text{p}_\mathcal{M}(X_3=1,X_4=0)$. The values of the leaf, sum and product nodes are given in brackets on their bottom, top and left respectively. The value of the root node is the answer to the query. (b) QPC obtained from the PC given in (a) for query variables $\{X_3,X_4\}$. For simplicity, here, we use a MMAP problem without any evidence. This is because a given evidence can be incorporated into the
PC by appropriately setting the leaf nodes. We also show value computations for the following leaf initialization: $X_3^c=0.99,\neg X_3^c=0.01, X_4^c=0.05,\neg X_4^c=0.95$ and all other leaves are set to $1$.}
    \label{fig:example}
\end{figure*}
We use upper case letters (e.g., $X$) to denote random variables and corresponding lower case letters (e.g., $x$) to denote an assignment of a value to a variable. We use bold upper case letters (e.g., $\mathbf{X}$) to denote a set of random variables and corresponding bold lower case letters (e.g., $\mathbf{x}$) to denote an assignment of values to all variables in the set. Given an assignment $\mathbf{x}$ to all variables in $\mathbf{X}$ and a variable $Y \in \mathbf{X}$, let $\mathbf{x}_Y$ denote the projection of $\mathbf{x}$ on $Y$. We assume that all random variables take values from the set $\{0, 1\}$; although note that it is easy to extend our method to multi-valued variables. 
%We use $\bar{X}$ to denote the complement of $X$. For any given integer $N$, we denote the set $\{1,\ldots,N\}$ by $[N]$.

\subsection{Probabilistic Circuits} 
A probabilistic circuit (PC) $\mathcal{M}$ \cite{choiProbCirc20} defined over a set of variables $\mathbf{X}$ represents a joint probability distribution over $\mathbf{X}$ using a rooted directed acyclic graph. The graph consists of three types of nodes: internal sum nodes that are labeled by $+$, internal product nodes that are labeled by $\times$, and leaf nodes that are labeled by either $X$ or $\neg X$ where $X \in \mathbf{X}$. Sum nodes represent conditioning, and an edge into a sum node $n$ from its child node $m$ is labeled by a real number $\omega(m,n)>0$. Given an internal node (either a sum or product node) $n$, let $\texttt{ch}(n)$ denote the set of children of $n$. We assume that each sum node $n$ is normalized and satisfies the following property: $\sum_{m\in \texttt{ch}(n)}\omega(m,n) = 1$. 


\eat{
The probability of an assignment $\mathbf{x}$ can be computed from $\mathcal{M}$ by appropriately assigning a value of $0$ or $1$ to each leaf node and then performing value computations over $\mathcal{M}$ via a bottom-up pass. Formally, given a node $n$, let $n(\mathbf{x})$ denote the value of $n$ given $\mathbf{x}$. Given $\mathbf{x}$, we initialize the value of each leaf node $n$ to $1$ iff the label of $n$ is $X$ and $X=1$ appears in $\mathbf{x}$ or the label of $n$ is $\neg X$ and $X=0$ appears in $\mathbf{x}$. Otherwise, we initialize the value of the leaf node to $0$. Then the value of each internal node $n$ is given by the following recursion:
\begin{align}
\label{eq:recursion}
    n(\mathbf{x}) = \left \{ \begin{array}{cc}
    \sum_{m \in \texttt{ch}(n)} \omega(m,n) m(\mathbf{x}) & \text{if $n$ is a sum node}\\
    \prod_{m \in \texttt{ch}(n)} m(\mathbf{x}) &\text{if $n$ is a product node}
    \end{array} \right .
\end{align}
Let $r_\mathcal{M}$ denote the root node of $\mathcal{M}$. Then, the probability of $\mathbf{x}$ w.r.t. $\mathcal{M}$, denoted by $\text{p}_\mathcal{M}(\mathbf{x})$ equals $r_\mathcal{M}(\mathbf{x})$. 
}


In this paper, we focus on a class of PCs which are \textit{smooth and decomposable} \cite{choiProbCirc20,NEURIPS2021_vergari}. Examples of such PCs include sum-product networks \cite{poon2011sum}, mixtures of cutset networks \cite{rahman2014cutset,rahman_cutsetnetworks_2016} and arithmetic circuits obtained by compiling probabilistic graphical models \cite{darwiche2003differential}. These PCs admit tractable marginal inference, a key property that we leverage in our proposed method.

\begin{definition}
We say that a sum or a product node $n$ is defined over a variable $X$ if there exists a directed path from $n$ to a leaf node labeled either by $X$ or $\neg X$. A PC is \textbf{\textit{smooth}} if each sum node is such that its children are defined over the same set of variables. A PC is \textbf{\textit{decomposable}} if each product node is such that its children are defined over disjoint subsets of variables.
\end{definition}

\begin{example}
Figure \ref{fig:example}(a) shows a smooth and decomposable probabilistic circuit defined over $\{X_1,\ldots,X_4\}$.
\end{example}

\subsection{Marginal Inference in PCs}
Next, we describe how to compute the probability of an assignment to a subset of variables in a smooth and decomposable PC. This task is called the marginal inference (\texttt{MAR}) task. We begin by describing some additional notation.

Given a PC $\mathcal{M}$ defined over $\mathbf{X}$, let $\mathcal{S}$, $\mathcal{P}$ and $\mathcal{L}$ denote the set of sum, product and leaf nodes of $\mathcal{M}$ respectively. Let $\mathbf{Q} \subseteq \mathbf{X}$. Given a node $n$ and an assignment $\mathbf{q}$, let $v(n,\mathbf{q})$ denote the value of $n$ given $\mathbf{q}$. Given a leaf node $n$, let $\texttt{var}(n)$ denote the variable associated with $n$ and let $l(n,\mathbf{q})$ be a function, which we call \textit{leaf function}, that is defined as follows. $l(n,\mathbf{q})$ equals $0$ if any of the following two conditions are satisfied: (1) the label of $n$ is $Q$ where $Q \in \mathbf{Q}$ and $\mathbf{q}$ contains the assignment $Q=0$; and (2) if the label of $n$ is $\neg Q$ and $\mathbf{q}$ contains the assignment $Q=1$. Otherwise, it is equal to $1$. Intuitively, the leaf function assigns all leaf nodes that are inconsistent with the assignment $\mathbf{q}$ to $0$ and the remaining nodes, namely those that are consistent with $\mathbf{q}$ and those that are not part of the query to $1$.

%Given a leaf node $n$, (1) let $\texttt{sign}(n)$ be a function that equals $1$ if $n$ is labeled by $X$ and equals $0$ if $n$ is labeled by $\neg X$, where $X \in \mathbf{X}$; (2) let $\texttt{var}(n)$ denote the variable associated with $n$; and (3) let $l(n,\mathbf{q})$ be a function, which we call leaf function, that is defined as follows. $l(n,\mathbf{q})$ equals $0$ if any of the following two conditions are satisfied: (1) the label of $n$ is $Q$ where $Q \in \mathbf{Q}$ and $\mathbf{q}$ contains the assignment $Q=0$; and (2) if the label of $n$ is $\neg Q$ and $\mathbf{q}$ contains the assignment $Q=1$. Otherwise, it is equal to $1$. 

%The marginal probability of any assignment $\mathbf{q}$ w.r.t $\mathcal{M}$, and denoted by $\text{p}_{\mathcal{M}}(\mathbf{q})$ can be computed by appropriately assigning a value of $0$ or $1$ to each leaf node and then performing recursive value computations over $\mathcal{M}$ via a bottom-up pass (and thus \texttt{MAR} inference is tractable or linear time in PCs). Formally, given a node $n$ and an assignment $\mathbf{q}$, let $v(n,\mathbf{q})$ denote the value of $n$ given $\mathbf{q}$. 



%$l(n,\mathbf{q})$ equals $(\mathbf{q}_{\texttt{var}(n)})^{\texttt{sign}(n)} \times (1-\mathbf{q}_{\texttt{var}(n)})^{(1-\texttt{sign}(n))}$ if $\texttt{var}(n) \in \mathbf{Q}$ and equals $1$ otherwise. At a high level, given $\mathbf{q}$ and a leaf node $n$, the leaf function outputs a $1$ if the label of $n$ is $Q$ where $Q \in \mathbf{Q}$ and $Q=1$ appears in $\mathbf{q}$ or if the label of $n$ is $\neg Q$ and $Q=0$ appears in $\mathbf{q}$. Otherwise, it outputs a $1$. 



\eat{
\begin{align}
    \label{eq:leaf-function}
    f(n,\mathbf{q}) = \left \{ \begin{array}{cc}
       (\mathbf{q}_{\texttt{var}(n)})^\texttt{sign}(n) \times (1-(\mathbf{q}_{\texttt{var}(n)})^{(1-\texttt{sign}(n))}  &  \text{if $\texttt{var}(n) \in \mathbf{Q}$}\\
       1  & \text{otherwise} 
    \end{array}\right .
\end{align}
}

%The probability of an assignment $\mathbf{x}$ can be computed from $\mathcal{M}$ by appropriately assigning a value of $0$ or $1$ to each leaf node and then performing value computations over $\mathcal{M}$ via a bottom-up pass. Formally, given a node $n$, let $n(\mathbf{x})$ denote the value of $n$ given $\mathbf{x}$. Given $\mathbf{x}$, we initialize the value of each leaf node $n$ to $1$ iff the label of $n$ is $X$ and $X=1$ appears in $\mathbf{x}$ or the label of $n$ is $\neg X$ and $X=0$ appears in $\mathbf{x}$. Otherwise, we initialize the value of the leaf node to $0$. Then 

%The marginal probability of any assignment $\mathbf{q}$ w.r.t $\mathcal{M}$, and denoted by $\text{p}_{\mathcal{M}}(\mathbf{q})$ can be computed by appropriately assigning a value of $0$ or $1$ to each leaf node and then performing recursive value computations over $\mathcal{M}$ via a bottom-up pass (and thus \texttt{MAR} inference is tractable or linear time in PCs). Under this notation, the value of each internal node $n$ is given by the following recursion:
Under this notation, and given a leaf function $l(n,\mathbf{q})$, the marginal probability of any assignment $\mathbf{q}$ w.r.t $\mathcal{M}$, and denoted by $\text{p}_{\mathcal{M}}(\mathbf{q})$ can be computed by performing the following recursive \textit{value computations}:
\begin{align}
\label{eq:recursion}
    v(n,\mathbf{q}) = \left \{ \begin{array}{ll}
    l(n,\mathbf{q}) & \text{if $n \in \mathcal{L}$}\\
    \sum_{m \in \texttt{ch}(n)} \omega(m,n) v(m,\mathbf{q}) & \text{if $n \in \mathcal{S}$}\\
    \prod_{m \in \texttt{ch}(n)} v(m,\mathbf{q}) &\text{if $n \in \mathcal{P}$}
    \end{array} \right .
\end{align}
Let $r$ denote the root node of $\mathcal{M}$. Then, the probability of $\mathbf{q}$ w.r.t. $\mathcal{M}$, denoted by $\text{p}_\mathcal{M}(\mathbf{q})$ equals $v(r,\mathbf{q})$. Note that if $\mathbf{Q}=\mathbf{X}$, then $v(r,\mathbf{x})$ denotes the probability of the joint assignment $\mathbf{x}$ to all variables in the PC. Thus
\[ v(r,\mathbf{q})= \sum_{\mathbf{y} \in \{0,1\}^{|\mathbf{Y}|}} v (r,(\mathbf{q},\mathbf{y})) \]
where $\mathbf{Y}=\mathbf{X} \setminus \mathbf{Q}$ and the notation $(\mathbf{q},\mathbf{y})$ denotes the \textit{composition} of the assignments to $\mathbf{Q}$ and $\mathbf{Y}$ respectively.

Since the recursive value computations require only one bottom-up pass over the PC, \texttt{MAR} inference is tractable or linear time in smooth and decomposable PCs.

%can be computed by making one bottom-up pass over the PC $\mathcal{M}$. 

\eat{The only thing that changes from the recursive method used to computed the probability of a joint assignment $\mathbf{x}$ is the initialization step. Here, we initialize all leaf nodes that are not associated with variables in $\mathbf{Q}$ to $1$. Then, given $\mathbf{q}$, we initialize the value of each leaf node $n$ to $1$ if the label of $n$ is $Q$ where $Q \in \mathbf{Q}$ and $Q=1$ appears in $\mathbf{q}$ or if the label of $n$ is $\neg Q$ where $Q \in \mathbf{Q}$ and $Q=0$ appears in $\mathbf{q}$. Otherwise, we set the value of the leaf node to $0$. Then, using the recursive procedure given in Eq. \eqref{eq:recursion} to compute the values of the nodes, the marginal probability $\text{p}_\mathcal{M}(\mathbf{q})$ equals the value of the root node $r_{\mathcal{M}}(\mathbf{q})$.}


\begin{example}
Figure \ref{fig:example}(a) shows bottom-up, recursive value computations for computing the probability of the assignment $(X_3=1,X_4=0)$ in our running example. Here, the leaf nodes $\neg X_3$ and $X_4$ are assigned to $0$ and all other leaf nodes are assigned to $1$. The number in brackets at the top, left and bottom of each sum, product and leaf nodes respectively shows the value of the corresponding node. The value of the root node equals $\text{p}_\mathcal{M}(X_3=1,X_4=0)$.
\end{example}
\subsection{Marginal maximum-a-posteriori (MMAP) Inference in PCs}
Given a PC $\mathcal{M}$ defined over $\mathbf{X}$, let $\mathbf{E} \subseteq \mathbf{X}$ and $\mathbf{Q} \subseteq \mathbf{X}$ denote the set of evidence and query variables respectively such that $\mathbf{E} \cap \mathbf{Q}=\emptyset$. Let $\mathbf{H}=\mathbf{X} \setminus (\mathbf{Q} \cup \mathbf{E})$ denote the set of hidden variables. Given an assignment $\mathbf{e}$ to the evidence variables (called evidence), the MMAP task seeks to find an assignment $\mathbf{q}$ to $\mathbf{Q}$ such that the probability of the assignment $(\mathbf{e},\mathbf{q})$ w.r.t. $\mathcal{M}$ is maximized. Mathematically, 
%The MMAP task is defined as follows. Given a PC $\mathcal{M}$ defined over $\mathbf{X}$, an assignment $\mathbf{e}$ (called evidence) to a subset of variables $\mathbf{E}$ (called evidence variables) and a subset $\mathbf{Q}$ (called query variables), we are interested in finding an assignment $\mathbf{q}$ to $\mathbf{Q}$ such that the probability of the assignment $(\mathbf{e},\mathbf{q})$ w.r.t. $\mathcal{M}$ is maximized. Mathematically, 
\begin{align}
\label{eqn:mmap}
\texttt{MMAP}(\mathbf{Q},\mathbf{e}) =& \argmax_{\mathbf{q}}  \text{p}_{\mathcal{M}}(\mathbf{e},\mathbf{q})\\ =& \argmax_{\mathbf{q}}  \sum_{\mathbf{h} \in \{0,1\}^{|\mathbf{H}|}}\text{p}_{\mathcal{M}}(\mathbf{e},\mathbf{q},\mathbf{h})
%=\argmax_{\mathbf{q}} v(r,(\mathbf{e},\mathbf{q}))
\end{align}
If $\mathbf{H} =\emptyset$ (namely $\mathbf{Q}$ is the set of non-evidence variables), then MMAP corresponds to the most probable explanation (MPE) task. It is known that both MMAP and MPE tasks are at least $NP$-hard in smooth and decomposable PCs \cite{park&darwiche04,decamposNewComplexityResultsMAPBayesianNetworks,conaty17,peharz2015foundations}, and even NP-hard to approximate \cite{conaty17,mei2018maximum}. 

A popular approach to solve the MMAP task in PCs is to replace the sum  ($\sum$) operator by the max operator during bottom-up, recursive value computations and then performing a second top-down pass to find the assignment \cite{poon2011sum}. 
%The subsets $\mathbf{E}$, $\mathbf{Q}$, and $\mathbf{H}$ are respectively called the sets of \textit{evidence}, \textit{query} and \textit{hidden} variables. 

\eat{Assuming $H$ is a latent class variable in example \ref{exmp:pc}, given evidence $\mathbf{E=e}$, the MMAP over the query variables $\mathbf{Q}$ can be found by solving the following multilinear program\footnote{\textcolor{red}{MMAP tasks can be formulated as integer linear programs (\cite{maua2020two}). We obtain linear programs by relaxing the integrality constraints.}}.
  \eat{  
    \begin{align*}  \argmax_{\mathbf{q}}\sum_{k\in[K]} \omega_k\bigg(\prod_{m\in[M]}(\alpha_{k,m}e_m+(1-\alpha_{k,m})(1 - e_m).\\
    \prod_{n\in[N]}(\beta_{k,n}q_n+(1-\beta_{k,n})(1-q_n)\bigg)
    \end{align*}
  }  
  }



==> content/related_work.tex <==
\eat{\section{Related Work}



Although PCs allow for tractable marginals and MPE computations \cite{rahmanNovelUpperBoundsConstrainedMostProbable, rouhaniAlgorithmsNearestAssignmentProblem2018}, solving the MMAP problem exactly is recognized as NP-Hard \cite{decamposNewComplexityResultsMAPBayesianNetworks}. This  complexity persists even when pursuing approximate solutions \cite{conaty17, mei2018maximum}. The significance of MMAP solvers lies in their potential utility across numerous real-world applications \cite{bioucasdiasBayesianImageSegmentationusinghiddenfields2016, kiselevPOMDPPlanningMarginalMAPProbabilisticInferenceGenerative, leeApplyingMarginalMapSearchProbabilisticConformantb}. \cite{maua2020two} focused on solving (M)MAP in sum-product networks (SPNs), a popular class of PCs with sophisticated deep architectures composed of layers of latent (mixture) variables. The authors proposed two approaches to reformulate MAP in SPNs. The first approach converts any SPN to an equivalent Bayesian network on which existing MAP solvers based on message-passing can be used. The second approach converts any SPN to a mixed integer linear program which can then be solved by off-the-shelf solvers. \cite{choi2022solving} proposed to solve MMAP exactly in PCs by iteratively pruning away irrelevant portions of the model until the MMAP solution can be read off easily. 

In the context of machine learning research, neural networks have emerged as versatile tools for addressing complex probabilistic inference tasks, including Maximum A Posteriori (MAP) and Most Probable Explanation (MPE) inference \cite{gilmerNeuralMessagePassingQuantumChemistry, kuckBeliefPropagationNeuralNetworks, NEURIPS2020_61c66a2f, satorrasNeuralEnhancedBeliefPropagationFactorGraphs}. However, many existing methods within this domain necessitate precise inference outcomes for training neural networks to handle future probabilistic queries effectively. Recently, \citet{cui_variational_2022} proposed a novel approach to address the MPE task. Their methodology introduces a self-supervised training paradigm wherein a neural network parameterizes a variational distribution. Numerous self-supervised methodologies within the learning to optimize domain \cite{fioretto_optimalpowerflows_2020,  donti_methodoptimizationhard_2020, zamzam_solutionsextremelyfast_2020, park_learningconstrainedoptimization_2023} leverage neural networks to address various optimization tasks.
}

==> content/tables/contingency-base.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[hbt!]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|cccc|cccc|}
\hline
    & \multicolumn{4}{c|}{MPE}                     & \multicolumn{4}{c|}{MMAP}                    \\ \cline{2-9} 
    & \spn & \cellcolor[HTML]{D4D4D4}\ourfig & \mle & \seq & \spn & \cellcolor[HTML]{D4D4D4}\ourfig & \mle & \seq \\ \hline
\spn & 0   & \cellcolor[HTML]{D4D4D4}64 & 33  & 14  & 0   & \cellcolor[HTML]{D4D4D4}46 & 23  & 10  \\
\rowcolor[HTML]{D4D4D4} 
\ourfig  & 88  & 0                          & 96  & 77  & 97  & 0                          & 102 & 82  \\
\mle & 6   & \cellcolor[HTML]{D4D4D4}49 & 0   & 15  & 3   & \cellcolor[HTML]{D4D4D4}34 & 0   & 10  \\
\seq & 105 & \cellcolor[HTML]{D4D4D4}63 & 105 & 0   & 117 & \cellcolor[HTML]{D4D4D4}53 & 117 & 0   \\ \hline
\end{tabular}%
}
\caption{Contingency tables over the competing methods for MPE and MMAP problems. The value in cell $(i,j)$ equals the number of times out of 154 that the scheme in the $i$-th row was better in terms of log-likelihood score than the scheme in the $j$-th column. Highlighted values represent results for the method proposed in this paper (\our).}
\label{tab:contingency-base}
\end{table}

==> content/tables/contingency-cifar-base.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{|cc
>{\columncolor[HTML]{D4D4D4}}c cc|}
\hline
                                & \spn                       & \ourfig & \mle                       & \seq                       \\ \hline
\spn                             & 0                         & 0       & 0                         & 2                         \\
\cellcolor[HTML]{D4D4D4}\ourfig & \cellcolor[HTML]{D4D4D4}9 & 0       & \cellcolor[HTML]{D4D4D4}9 & \cellcolor[HTML]{D4D4D4}9 \\
\mle                             & 0                         & 0       & 0                         & 2                         \\
\seq                             & 7                         & 0       & 7                         & 0                         \\ \hline
\end{tabular}%
}
\caption{Contingency tables over the competing methods for MPE on the CIFAR-10 dataset. Highlighted values represent results for the method proposed in this paper (\our).}
\label{tab:cifar10-base}
\end{table}

==> content/tables/contingency-hill-climbing.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[hbt!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|cccc|cccc|}
\hline
                   & \multicolumn{4}{c|}{MPE}                                 & \multicolumn{4}{c|}{MMAP}                                \\ \cline{2-9} 
\multirow{-2}{*}{} & \spn & \cellcolor[HTML]{D4D4D4}\ourfig & \mle & \seq & \spn & \cellcolor[HTML]{D4D4D4}\ourfig & \mle & \seq \\ \cline{2-9} 
\spn             & 0      & \cellcolor[HTML]{D4D4D4}40    & 13     & 9      & 0      & \cellcolor[HTML]{D4D4D4}27    & 10     & 16     \\
\rowcolor[HTML]{D4D4D4} 
\ourfig              & 93     & 0                             & 99     & 87     & 98     & 0                             & 100    & 86     \\
\mle             & 19     & \cellcolor[HTML]{D4D4D4}37    & 0      & 14     & 12     & \cellcolor[HTML]{D4D4D4}26    & 0      & 17     \\
\seq             & 85     & \cellcolor[HTML]{D4D4D4}44    & 82     & 0      & 89     & \cellcolor[HTML]{D4D4D4}39    & 90     & 0      \\ \hline
\end{tabular}%
}
\caption{Contingency tables for Hill Climbing Search initialized using the competing methods for MPE and MMAP problems. Highlighted values represent results for the method proposed in this paper (\our)}%.Method Comparison for Hill Climbing Search with Varied Initializations in MPE and MMAP Problems with Superiority Counts. Highlighted Values Indicate Proposed Method Comparisons.}
\label{tab:contingency-hill}
\end{table}

==> content/tables/contingency-mnist-emnist-base.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|cccc|cccc|}
\hline
        & \multicolumn{4}{c|}{MNIST}                                                                                                         & \multicolumn{4}{c|}{EMNIST}                                                                                                        \\ \cline{2-9} 
        & \multicolumn{1}{c}{\spn} & \multicolumn{1}{c}{\cellcolor[HTML]{D4D4D4}\ourfig} & \multicolumn{1}{c}{\mle} & \multicolumn{1}{c|}{\seq} & \multicolumn{1}{c}{\spn} & \multicolumn{1}{c}{\cellcolor[HTML]{D4D4D4}\ourfig} & \multicolumn{1}{c}{\mle} & \multicolumn{1}{c|}{\seq} \\ \hline
\spn     & 0                       & \cellcolor[HTML]{D4D4D4}1                           & 0                       & 1                        & 0                       & \cellcolor[HTML]{D4D4D4}1                           & 0                       & 5                        \\
\rowcolor[HTML]{D4D4D4} 
\ourfig & 9                       & 0                                                   & 9                       & 9                        & 7                       & 0                                                   & 7                       & 7                        \\
\mle     & 0                       & \cellcolor[HTML]{D4D4D4}1                           & 0                       & 1                        & 0                       & \cellcolor[HTML]{D4D4D4}1                           & 0                       & 5                        \\
\seq     & 9                       & \cellcolor[HTML]{D4D4D4}1                           & 9                       & 0                        & 3                       & \cellcolor[HTML]{D4D4D4}1                           & 3                       & 0                        \\ \hline
\end{tabular}%
}
\caption{Contingency tables over the competing methods for MPE on the MNIST and EMNIST datasets. Highlighted values represent results for the method proposed in this paper.}%Comparison of Methods MNIST and EMNIST Datasets for MPE with Method Superiority. Highlighted Values Indicate Proposed Method Comparisons.}
\label{tab:mnist-base}
\end{table}

==> content/tables/old/contingency_emnist-base.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllllll}
\hline
         & SPN & \ourfig & \ourfig+Train & \ourfig+Ent & MLE & Seq \\ \hline
SPN      & 0   & 1  & 1        & 3      & 0   & 5   \\
NN       & 7   & 0  & 0        & 5      & 7   & 7   \\
NN+Train & 7   & 3  & 0        & 4      & 7   & 7   \\
NN+Ent   & 5   & 3  & 4        & 0      & 5   & 5   \\
MLE      & 0   & 1  & 1        & 3      & 0   & 5   \\
Seq      & 3   & 1  & 1        & 3      & 3   & 0   \\ \hline
\end{tabular}%
}
\caption{Comparison Table for EMNIST Dataset: Method Superiority without Dataset Variables in $H$}
\label{tab:contingency-emnist-base}
\end{table}

==> content/tables/old/contingency_mmap-base.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllllll@{}}
\toprule
         & SPN & \ourfig & \ourfig+Train & \ourfig+Ent & MLE & Seq \\ \midrule
SPN      & 0   & 46 & 42       & 44     & 23  & 10  \\
NN       & 97  & 0  & 0        & 69     & 102 & 82  \\
NN+Train & 105 & 51 & 0        & 73     & 109 & 88  \\
NN+Ent   & 104 & 65 & 65       & 0      & 108 & 85  \\
MLE      & 3   & 34 & 31       & 33     & 0   & 10  \\
Seq      & 117 & 53 & 51       & 55     & 117 & 0   \\ \bottomrule
\end{tabular}
}
\caption{Contingency table showing method comparisons when dataset variables are included in $H$, indicating method superiority counts.}
\label{tab:contingency-mmap-base}
\end{table}

==> content/tables/old/contingency_mmap-search.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
       & SPN+HC & \ourfig+HC & MLE+HC & Seq+HC \\ \midrule
SPN+HC & 0      & 27    & 10     & 16     \\
NN+HC  & 98     & 0     & 100    & 86     \\
MLE+HC & 12     & 26    & 0      & 17     \\
Seq+HC & 89     & 39    & 90     & 0      \\ \bottomrule
\end{tabular}%
}
\caption{Contingency table for Hill Climbing search with varied initializations, comparing results when dataset variables are included in $H$, showing method superiority counts.}
\label{tab:contingency-mmap-search}
\end{table}

==> content/tables/old/contingency_mnist-base.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllllll}
\hline
         & SPN & \ourfig & \ourfig+Train & \ourfig+Ent & MLE & Seq \\ \hline
SPN      & 0   & 1  & 1        & 2      & 0   & 1   \\
NN       & 9   & 0  & 0        & 7      & 9   & 9   \\
NN+Train & 9   & 9  & 0        & 8      & 9   & 9   \\
NN+Ent   & 8   & 3  & 2        & 0      & 8   & 8   \\
MLE      & 0   & 1  & 1        & 2      & 0   & 1   \\
Seq      & 9   & 1  & 1        & 2      & 9   & 0   \\ \hline
\end{tabular}%
}
\caption{Comparison Table for MNIST Dataset: Method Superiority without Dataset Variables in $H$}
\label{tab:contingency-mnist-base}
\end{table}

==> content/tables/old/contingency_mpe-base.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllllll@{}}
\toprule
         & SPN & \ourfig & \ourfig+T & \ourfig+E & MLE & Seq \\ \midrule
SPN      & 0   & 64 & 61       & 74     & 33  & 14  \\
NN       & 88  & 0  & 0        & 115    & 96  & 77  \\
NN+Train & 91  & 50 & 0        & 94     & 98  & 80  \\
NN+Ent   & 74  & 33 & 47       & 0      & 81  & 68  \\
MLE      & 6   & 49 & 47       & 60     & 0   & 15  \\
Seq      & 105 & 63 & 59       & 67     & 105 & 0   \\ \bottomrule
\end{tabular}
}
\caption{Contingency table showing method comparisons when dataset variables aren't in $H$, indicating method superiority counts.}
\label{tab:contingency-mpe-base}
\end{table}



==> content/tables/old/contingency_mpe-search.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
\label{tab:contingency-mpe-search}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
       & SPN+HC & \ourfig+HC & MLE+HC & Seq+HC \\ \midrule
SPN+HC & 0      & 40    & 13     & 9      \\
NN+HC  & 93     & 0     & 99     & 87     \\
MLE+HC & 19     & 37    & 0      & 14     \\
Seq+HC & 85     & 44    & 82     & 0      \\ \bottomrule
\end{tabular}%
}
\caption{Contingency table for Hill Climbing search with different initializations, comparing results without dataset variables in $H$, indicating method superiority counts.}
\end{table}

==> content/tmp-related.tex <==
\section{Related Work}
\cite{peharz2015foundations} and \cite{conaty17} showed that 

Prior work, primarily in the graphical models literature demonstrated that the MMAP problem has numerous real-world applications, especially in health care, linkage analysis and diagnosis where hidden variables are present and need to be marginalized out \cite{bioucasdiasBayesianImageSegmentationusinghiddenfields2016, kiselevPOMDPPlanningMarginalMAPProbabilisticInferenceGenerative, leeApplyingMarginalMapSearchProbabilisticConformantb,NIPS2015_faacbcd5}. In terms of computational complexity, \cite{park&darwiche04} showed that MMAP inference is $NP^{PP}$-hard in arbitrary graphical models and their results were further extended by \cite{decamposNewComplexityResultsMAPBayesianNetworks}. \cite{peharz2015foundations} showed that MMAP/MPE inference is NP-hard in 


Although PCs allow for tractable marginals and MPE computations \cite{rahmanNovelUpperBoundsConstrainedMostProbable, rouhaniAlgorithmsNearestAssignmentProblem2018}, solving the MMAP problem exactly is recognized as NP-Hard \cite{decamposNewComplexityResultsMAPBayesianNetworks}. This  complexity persists even when pursuing approximate solutions \cite{conaty17, mei2018maximum}. The significance of MMAP solvers lies in their potential utility across numerous real-world applications \cite{bioucasdiasBayesianImageSegmentationusinghiddenfields2016, kiselevPOMDPPlanningMarginalMAPProbabilisticInferenceGenerative, leeApplyingMarginalMapSearchProbabilisticConformantb}. \cite{maua2020two} focused on solving (M)MAP in sum-product networks (SPNs), a popular class of PCs with sophisticated deep architectures composed of layers of latent (mixture) variables. The authors proposed two approaches to reformulate MAP in SPNs. The first approach converts any SPN to an equivalent Bayesian network on which existing MAP solvers based on message-passing can be used. The second approach converts any SPN to a mixed integer linear program which can then be solved by off-the-shelf solvers. \cite{choi2022solving} proposed to solve MMAP exactly in PCs by iteratively pruning away irrelevant portions of the model until the MMAP solution can be read off easily. 

In the context of machine learning research, neural networks have emerged as versatile tools for addressing complex probabilistic inference tasks, including Maximum A Posteriori (MAP) and Most Probable Explanation (MPE) inference \cite{gilmerNeuralMessagePassingQuantumChemistry, kuckBeliefPropagationNeuralNetworks, NEURIPS2020_61c66a2f, satorrasNeuralEnhancedBeliefPropagationFactorGraphs}. However, many existing methods within this domain necessitate precise inference outcomes for training neural networks to handle future probabilistic queries effectively. Recently, \citet{cui_variational_2022} proposed a novel approach to address the MPE task. Their methodology introduces a self-supervised training paradigm wherein a neural network parameterizes a variational distribution. Numerous self-supervised methodologies within the learning to optimize domain \cite{fioretto_optimalpowerflows_2020,  donti_methodoptimizationhard_2020, zamzam_solutionsextremelyfast_2020, park_learningconstrainedoptimization_2023} leverage neural networks to address various optimization tasks.

==> figures/pc1.tex <==
% \documentclass[tikz]{standalone}
% \usepackage{tikz}
% \newcommand{\myscale}{0.02}
% \usetikzlibrary{positioning,quotes}
% \newcommand{\eat}[1]{}
% \begin{document}
    \begin{tikzpicture}[thick,scale=\myscale]
    \node[circle,draw,label=north:({\footnotesize 0.0778})](r) {$+$};
    \node[circle,draw](l11) [below left = of r,label=west:({\footnotesize 0.026})] {$\times$};
    \node[circle,draw](l12) [below right = of r,label=west:({\footnotesize 0.1})] {$\times$};
    \node(l21) [below left = of l11,label=south:({\footnotesize 1})] {$X_1$};
    \node[circle,draw](l22) [below  = of l11,label=north:({\footnotesize 0.026})] {$+$};
    \node[circle,draw](l23) [below = of l12,,label=north:({\footnotesize 0.1})] {$+$};
    \node(l24) [below right = of l12,label=south:({\footnotesize 1})] {$\neg X_1$};
    \node[circle,draw](l31) [below left = of l22,label=west:({\footnotesize 0.03})] {$\times$};
    \node[circle,draw](l32) [below left = of l23,label=west:({\footnotesize 0.02})] {$\times$};
    \node[circle,draw](l33) [below right = of l23,label=west:({\footnotesize 0.12})] {$\times$};
    \node[circle,draw](l41) [below left = of l31,label=north:({\footnotesize 0.3})] {$+$};
    \node(l42) [below  = of l31,label=south:({\footnotesize 1})] {$\neg X_2$};
    \node[circle,draw](l43) [right = of l42,label=north:({\footnotesize 0.1})] {$+$};
    \node(l44) [right = of l43,label=south:({\footnotesize 1})] {$X_2$};
    \node[circle,draw](l45) [right = of l44,label=north:({\footnotesize 0.2})] {$+$};
    \node(l46) [right = of l45,label=south:({\footnotesize 1})] {$\neg X_2$};
    \node[circle,draw](l47) [right = of l46,label=north:({\footnotesize 0.6})] {$+$};
    \node(l51) [below left = of l41,label=south:({\footnotesize 1})] {$X_3$};
    \node(l52) [right  = of l51,label=south:({\footnotesize 0})] {$\neg X_3$};
    \node(l53) [right = of l52,label=south:({\footnotesize 0})] {$X_4$};
    \node(l54) [right = of l53,label=south:({\footnotesize 1})] {$\neg X_4$};
    \node(l55) [right = of l54,label=south:({\footnotesize 1})] {$X_3$};
    \node(l56) [right = of l55,label=south:({\footnotesize 0})] {$\neg X_3$};
    \node(l57) [right = of l56,label=south:({\footnotesize 0})] {$X_4$};
    \node(l58) [right = of l57,label=south:({\footnotesize 1})] {$\neg X_4$};
    
    \draw[->] (r) edge node[left]{$0.3$} (l11);
    \draw[->] (r) edge node[right]{$0.7$}(l12);
    \draw[->] (l11) edge (l21);
    \draw[->] (l11) edge (l22);
    \draw[->] (l12) edge (l23);
    \draw[->] (l12) edge (l24);
    \draw[->] (l22) edge node[left]{$0.6$} (l31);
    \draw[->] (l22) edge node[right]{$0.4$} (l32);
    \draw[->] (l23) edge node[left]{$0.2$}(l32);
    \draw[->] (l23) edge node[right]{$0.8$} (l33);

    \draw[->] (l31) edge (l41);
    \draw[->] (l31) edge (l42);
    \draw[->] (l31) edge (l43);

    \draw[->] (l32) edge (l43);
    \draw[->] (l32) edge (l44);
    \draw[->] (l32) edge (l45);

    \draw[->] (l33) edge (l45);
    \draw[->] (l33) edge (l46);
    \draw[->] (l33) edge (l47);

    \draw[->] (l41) edge node[left]{$0.3$}(l51);
    \draw[->] (l41) edge node[right]{$0.7$}(l52);
    \draw[->] (l43) edge node[left]{$0.9$}(l53);
    \draw[->] (l43) edge node[right]{$0.1$}(l54);
    \draw[->] (l45) edge node[left]{$0.2$}(l55);
    \draw[->] (l45) edge node[right]{$0.8$}(l56);
    \draw[->] (l47) edge node[left]{$0.4$}(l57);
    \draw[->] (l47) edge node[right]{$0.6$}(l58);
    \eat{
    \node(r) at (0,6) {$+$};
    \node(l1) at (1,5){$\times$};
    \node(l1) at (1,7){$\times$};
    }
    \eat{
    \node (a) {$A$};
    \node (z) [right = of a] {$Z$};
    \node (b) [right = of z] {$B$};
    \node (x) [below left = of z] {$X$};
    \node (y) [below right = of z] {$Y$};
    \node (c) [below right = of x] {$C$};
    \path (a) edge (x);
    \path (a) edge (z);
    \path (b) edge (y);
    \path (b) edge (z);
    \path (c) edge (x);
    \path (c) edge (y);
    \path (x) edge (y);
    \path (z) edge (x);
    \path (z) edge (y); 
    }
    \end{tikzpicture}
% \end{document}

==> figures/pc2.tex <==
% \documentclass[tikz]{standalone}
% \usepackage{tikz}
% \newcommand{\myscale}{0.02}
% \usetikzlibrary{positioning,quotes}
% \newcommand{\eat}[1]{}
% \begin{document}
    \begin{tikzpicture}[thick,scale=\myscale]
    \node[circle,draw,label=north:({\footnotesize 0.0832})](r) {$+$};
    \node[circle,draw](l11) [below left = of r,label=west:({\footnotesize 0.03707})] {$\times$};
    \node[circle,draw](l12) [below right = of r,label=west:({\footnotesize 0.103})] {$\times$};
    \node(l21) [below left = of l11,label=south:({\footnotesize 1})] {$X_1$};
    \node[circle,draw](l22) [below  = of l11,label=north:({\footnotesize 0.03707})] {$+$};
    \node[circle,draw](l23) [below = of l12,,label=north:({\footnotesize 0.103})] {$+$};
    \node(l24) [below right = of l12,label=south:({\footnotesize 1})] {$\neg X_1$};
    \node[circle,draw](l31) [below left = of l22,label=west:({\footnotesize 0.04256})] {$\times$};
    \node[circle,draw](l32) [below left = of l23,label=west:({\footnotesize 0.02884})] {$\times$};
    \node[circle,draw](l33) [below right = of l23,label=west:({\footnotesize 0.1215})] {$\times$};
    \node[circle,draw](l41) [below left = of l31,label=north:({\footnotesize 0.304})] {$+$};
    \node(l42) [below  = of l31,label=south:({\footnotesize 1})] {$\neg X_2$};
    \node[circle,draw](l43) [right = of l42,label=north:({\footnotesize 0.14})] {$+$};
    \node(l44) [right = of l43,label=south:({\footnotesize 1})] {$X_2$};
    \node[circle,draw](l45) [right = of l44,label=north:({\footnotesize 0.206})] {$+$};
    \node(l46) [right = of l45,label=south:({\footnotesize 1})] {$\neg X_2$};
    \node[circle,draw](l47) [right = of l46,label=north:({\footnotesize 0.59})] {$+$};
    \node(l51) [below left = of l41,label=south:({\footnotesize 0.99})] {$X_3^c$};
    \node(l52) [right  = of l51,label=south:({\footnotesize 0.01})] {$\neg X_3^c$};
    \node(l53) [right = of l52,label=south:({\footnotesize 0.05})] {$X_4^c$};
    \node(l54) [right = of l53,label=south:({\footnotesize 0.95})] {$\neg X_4^c$};
    \node(l55) [right = of l54,label=south:({\footnotesize 0.99})] {$X_3^c$};
    \node(l56) [right = of l55,label=south:({\footnotesize 0.01})] {$\neg X_3^c$};
    \node(l57) [right = of l56,label=south:({\footnotesize 0.05})] {$X_4^c$};
    \node(l58) [right = of l57,label=south:({\footnotesize 0.95})] {$\neg X_4^c$};
    
    \draw[->] (r) edge node[left]{$0.3$} (l11);
    \draw[->] (r) edge node[right]{$0.7$}(l12);
    \draw[->] (l11) edge (l21);
    \draw[->] (l11) edge (l22);
    \draw[->] (l12) edge (l23);
    \draw[->] (l12) edge (l24);
    \draw[->] (l22) edge node[left]{$0.6$} (l31);
    \draw[->] (l22) edge node[right]{$0.4$} (l32);
    \draw[->] (l23) edge node[left]{$0.2$}(l32);
    \draw[->] (l23) edge node[right]{$0.8$} (l33);

    \draw[->] (l31) edge (l41);
    \draw[->] (l31) edge (l42);
    \draw[->] (l31) edge (l43);

    \draw[->] (l32) edge (l43);
    \draw[->] (l32) edge (l44);
    \draw[->] (l32) edge (l45);

    \draw[->] (l33) edge (l45);
    \draw[->] (l33) edge (l46);
    \draw[->] (l33) edge (l47);

    \draw[->] (l41) edge node[left]{$0.3$}(l51);
    \draw[->] (l41) edge node[right]{$0.7$}(l52);
    \draw[->] (l43) edge node[left]{$0.9$}(l53);
    \draw[->] (l43) edge node[right]{$0.1$}(l54);
    \draw[->] (l45) edge node[left]{$0.2$}(l55);
    \draw[->] (l45) edge node[right]{$0.8$}(l56);
    \draw[->] (l47) edge node[left]{$0.4$}(l57);
    \draw[->] (l47) edge node[right]{$0.6$}(l58);
    \eat{
    \node(r) at (0,6) {$+$};
    \node(l1) at (1,5){$\times$};
    \node(l1) at (1,7){$\times$};
    }
    \eat{
    \node (a) {$A$};
    \node (z) [right = of a] {$Z$};
    \node (b) [right = of z] {$B$};
    \node (x) [below left = of z] {$X$};
    \node (y) [below right = of z] {$Y$};
    \node (c) [below right = of x] {$C$};
    \path (a) edge (x);
    \path (a) edge (z);
    \path (b) edge (y);
    \path (b) edge (z);
    \path (c) edge (x);
    \path (c) edge (y);
    \path (x) edge (y);
    \path (z) edge (x);
    \path (z) edge (y); 
    }
    \end{tikzpicture}
% \end{document}
